Budget Sharing for Multi-Analyst Differential Privacy

Large organizations that collect data about populations (like the US Census Bureau) release summary statistics that are used by multiple stakeholders for resource allocation and policy making problems. These organizations are also legally required to protect the privacy of individuals from whom they collect data. Differential Privacy (DP) provides a solution to release useful summary data while preserving privacy. Most DP mechanisms are designed to answer a single set of queries. In reality, there are often multiple stakeholders that use a given data release and have overlapping but not-identical queries. This introduces a novel joint optimization problem in DP where the privacy budget must be shared among different analysts. We initiate study into the problem of DP query answering across multiple analysts. To capture the competing goals and priorities of multiple analysts, we formulate three desiderata that any mechanism should satisfy in this setting -- The Sharing Incentive, Non-Interference, and Adaptivity -- while still optimizing for overall error. We demonstrate how existing DP query answering mechanisms in the multi-analyst settings fail to satisfy at least one of the desiderata. We present novel DP algorithms that provably satisfy all our desiderata and empirically show that they incur low error on realistic tasks.

==> AlgosBox.tex <==



% GENERIC VERSION
\dap{Right now this still uses the matrix notation for the Select Measure Reconstruct paradigm but has a generic selection step. Do we want to shif this to generic versions of all the steps? }




 % Independent Mechanism
\begin{algorithm}[h]
\SetAlgoLined
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
\Input{Set of $K$ workloads  $\mathbf{W} \leftarrow \{W_1, W_2 \dots W_k\ \} $,\\ 
Set of $K$ weights  $S \leftarrow \{s_1, s_2 \dots s_k\ \} $ , \\
Data vector $\mathbf{x}$,\\
privacy budget $\epsilon$,\\
Selection Mechanism $\mathcal{M}$} 
\Output{Answer vector ans}
\vspace{3 mm}
 \nonl \textbf{Selection Step} \\
 $\mathbf{A} \leftarrow \{\mathcal{M}(W_i) | W_i \in \mathbf{W}\}$\\
\vspace{3 mm}
\nonl \textbf{Measure step} \\

$\mathbf{a} \leftarrow \{A_i\mathbf{ x}| A_i \in \mathbf{ A} \}$\\
$\mathbf{y} \leftarrow \{a_i + \text{Lap}(k\norm{A_i}_1/s_i\epsilon) | \mathbf{a_i\in \mathbf{a}, s_i \in \mathbf{s}, A_i \in \mathbf{A}} \}$\\

\vspace{3 mm}
\nonl \textbf{Reconstruct step} \\
$\mathbf{\Bar{x}} \leftarrow \{\mathbf{A_i^+} y_i|A_i \in A ,  y_i \in y \}$ \\
ans $\leftarrow \{W_i \Bar{x}| W_i \in \mathbf{W}\}$\\
\vspace{3 mm }

\Return ans
 \caption{Independent Mechanism}
\end{algorithm}


%Weighted utilitarian Mechanism
\begin{algorithm}[h]
\SetAlgoLined
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
\Input{Set of $K$ workloads  $\mathbf{W} \leftarrow \{W_1, W_2 \dots W_k\ \} $,\\ 
Set of $K$ weights  $S \leftarrow \{s_1, s_2 \dots s_k\ \} $ , \\
Data vector $\mathbf{x}$,\\
privacy budget $\epsilon$,\\
Selection Mechanism $\mathcal{M}$}  
\Output{Answer vector ans}
\vspace{3 mm}

 \nonl \textbf{Selection Step} \\
  $\mathbf{\Tilde{A}} \leftarrow  \{\mathcal{M}(W_i) | W_i \in \mathbf{W}\}$\\ 
  
  $\mathbf{W'} \leftarrow  \{(s_i/ k)^2 \norm{W_i\Tilde{A^+_i}}_F^2 W_i | W_i \in \mathbf{W}, \Tilde{A_i} \in \mathbf{\Tilde{A}}\}$\\ 
 $\mathbf{A} \leftarrow \mathcal{M}(\mathbf{W'}) $\\
\vspace{3 mm}

\nonl \textbf{Measure step} \\

$\mathbf{a} \leftarrow \mathbf{Ax}$\\
$y \leftarrow \mathbf{a} + \text{Lap}(\norm{A}_1/\epsilon)$\\

\vspace{3 mm}
\nonl \textbf{Reconstruct step} \\
$\mathbf{\Bar{x}} \leftarrow \mathbf{A^+} y$\\
ans $\leftarrow \{W_i \Bar{x}| W_i \in \mathbf{W}\}$\\
\vspace{3 mm }

\Return ans
 \caption{Weighted Utilitarian Mechanism}
\end{algorithm}

%utilitarian Mechanism
\begin{algorithm}[h]
\SetAlgoLined
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
\Input{Set of $K$ workloads  $\mathbf{W} \leftarrow \{W_1, W_2 \dots W_k\ \} $,\\ 
Set of $K$ weights  $S \leftarrow \{s_1, s_2 \dots s_k\ \} $ , \\
Data vector $\mathbf{x}$,\\
privacy budget $\epsilon$,\\
Selection Mechanism $\mathcal{M}$} 
\Output{Answer vector ans}
\vspace{3 mm}

 \nonl \textbf{Selection Step} \\
  $\mathbf{W'} \leftarrow  \{W_i| W_i \in \mathbf{W}\}$\\ 
 $\mathbf{A} \leftarrow \mathcal{M}(\mathbf{W'}) $\\
\vspace{3 mm}

\nonl \textbf{Measure step} \\

$\mathbf{a} \leftarrow \mathbf{Ax}$\\
$y \leftarrow \mathbf{a} + \text{Lap}(\norm{A}_1/\epsilon)$\\

\vspace{3 mm}
\nonl \textbf{Reconstruct step} \\
$\mathbf{\Bar{x}} \leftarrow \mathbf{A^+} y$\\
ans $\leftarrow \{W_i \Bar{x}| W_i \in \mathbf{W}\}$\\
\vspace{3 mm }

\Return ans
 \caption{Utilitarian Mechanism}
\end{algorithm}



% Waterfilling Mechanism
\begin{algorithm}[h]
\SetAlgoLined
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
\Input{Set of $K$ workloads  $\mathbf{W} \leftarrow \{W_1, W_2 \dots W_k\ \} $,\\ 
Set of $K$ weights  $S \leftarrow \{s_1, s_2 \dots s_k\ \} $ , \\
Data vector $\mathbf{x}$,\\
privacy budget $\epsilon$,\\
Selection Mechanism $\mathcal{M}$} 
\Output{Answer vector ans}
\vspace{3 mm}

 \nonl \textbf{Selection Step} \\
 $\mathbf{A} \leftarrow \{\mathcal{M}(W_i) | W_i \in \mathbf{W}\}$\\
\vspace{3 mm}


 \nonl \textbf{Aggregation step}\\ 
 buckets $B \leftarrow \{\}$\\
 \For{$A_i \in \mathbf{A}$}{
    \For{$v_i \in A_i$}{
    $e = v_i/ \norm{v_i} $ \\
        \eIf{$e \in B$}{
            $B(e) += ||v_i||$
                         }{
                $B(e) = ||v_i|| $
            }
        }
     } 
     $\mathbf{A'} = \{c \cdot e | (e, c) \in B \} $
     \vspace{3 mm}
     
\nonl \textbf{Measure step} \\

$\mathbf{a} \leftarrow \mathbf{A'x}$\\
$y \leftarrow \mathbf{a} + \text{Lap}(\norm{A}_1/\epsilon)$\\

\vspace{3 mm}
\nonl \textbf{Reconstruct step} \\
$\mathbf{\Bar{x}} \leftarrow \mathbf{A'^+} y$\\
ans $\leftarrow \{W_i \Bar{x}| W_i \in \mathbf{W}\}$\\
\vspace{3 mm }

\Return ans
 \caption{Waterfilling Mechanism}
\end{algorithm}

%Identity 
\begin{algorithm}[h]
\SetAlgoLined
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
\Input{Set of $K$ workloads  $\mathbf{W} \leftarrow \{W_1, W_2 \dots W\ \} $ , Data vector $\mathbf{x}$, privacy budget $\epsilon$} 
\Output{Answer vector ans}
\vspace{3 mm}

 \nonl \textbf{Selection Step} \\
 $\mathbf{A} \leftarrow \text{Identity}(n)$

\nonl \textbf{Measure step} \\

$\mathbf{a} \leftarrow \mathbf{Ax}$\\
$y \leftarrow \mathbf{a} + \text{Lap}(1/\epsilon)$\\

\vspace{3 mm}
\nonl \textbf{Reconstruct step} \\
$\mathbf{\Bar{x}} \leftarrow \mathbf{A^+} y$\\
ans $\leftarrow \{W_i \Bar{x}| W_i \in \mathbf{W}\}$\\
\vspace{3 mm }

\Return ans
 \caption{Identity}
\end{algorithm}

==> Notes.tex <==
% This is a page for proofs and concepts in progress and is left as a working idea
\subsection{Definitions }
First lets note some notation $\mathbf{W}$ denotes a workload. $\mathcal{W}$ denotes a set of workloads, $ \mathcal{M}$ denotes a mechanism and each mechanism takes in as input a non-empty set of workloads and a value $\epsilon$
\begin{definition}[Non-interference]
Let $Err_i$ be the expected error of analyst $i$. 
% Note I need a decent way to introduce alternative workload notation
A mechanism $\mathcal{M}$ satisfies Non-Interference if for every analyst $i$ with preference workload $W_i$  there does not exist an alternative workload $W_i'$ where $Err_i(\mathcal{M}(\epsilon, \mathcal{W})) > Err_i(\mathcal{M}(\epsilon, \mathcal{W}'))$ and for at least one other analyst $j \neq i$ $Err_j(\mathcal{M}(\epsilon, \mathcal{W})) < Err_j(\mathcal{M}(\epsilon, \mathcal{W}'))$
\end{definition}
\begin{definition}[Sharing incentive]
Let $Err_i$ be the expected error of analyst $i$ and let $\mathcal{W}$ be the set of all analysts workloads.
% Note I need a decent way to introduce alternative workload notation
A mechanism $\mathcal{M}$ satisfies the Sharing Incentive if for every analyst $i$ the following holds. $$Err_i(\mathcal{M}(\epsilon,\mathcal{W})) \leq  Err_i(\mathcal{M}(\frac{\epsilon}{k},\{\mathbf{W}_i\}))$$

\end{definition}



\subsection{Rolling example}

\subsection{Proofs work}

\subsubsection{Independent Workload strategy Sharing incentive}
By using formula for the expected error of the matrix mechanism we get that the error for each analyst using the independent workload strategy is as follows. $$\frac{2}{(\epsilon/k)^2} \|\mathbf{W}_i \|^2_1 \|\mathbf{W_iW_i}^+ \|^2_F = \frac{2n}{(\epsilon / k)^2} \|\mathbf{W}_i \|^2_1 $$
We'll use that in later proofs. 
Trivially the independent workload strategy satisfies the Sharing Incentive since it's error is exactly equivalent to that if the analyst used the mechanism on their own.

\subsubsection{Unified workload strategy Sharing Incentive}
When an analyst does unified workload strategy on their own they get the exact same expected error as the independent case since the unified workload strategy is identical to the independent workload strategy when there is only one analyst. The same follows for the weighted unified workload strategy as shown bellow. \\
Let $\mathbf{W_i'}$ be the weighted query matrix of analyst $i$ which is weighted by a scale of $\frac{1}{x}$. Then when separating and computing on their own the expected error is as follows. 

$$\frac{2}{(\epsilon/k)^2} \|\mathbf{W}_i' \|^2_1 \|\mathbf{W_iW_i'}^+ \|^2_F] =$$ $$ \frac{2}{(\epsilon/k)^2} \|\frac{1}{x} \mathbf{W}_i \|^2_1 \|\mathbf{x W_iW_i}^+ \|^2_F]  =$$ $$ \frac{2}{(\epsilon/k)^2} \|\mathbf{W}_i \|^2_1 \frac{nx^2}{x^2} = \frac{2n}{(\epsilon/k)^2} \|\mathbf{W}_i \|^2_1 
$$

For both of those mechanisms consider the best case scenario where all analysts have the same workload. We note that then the unified workload is exactly the workload proposed by each analyst and we get the following expected error for each analyst.  $$\frac{2n}{\epsilon^2} \|\mathbf{W}_i \|^2_1  $$ 
Which is simply the independent case but with the entirety of the privacy budget. Note that we have also just proved that scaling the strategy matrix by some arbitrary constant doesn't change the error. This intuitively makes sense since if every analyst wants the same workload we might as well just compute answers for that one workload and give it to each of the analysts. We can use this as a lower bound for error for now, saying that at best in the unified case without scaling we can get error that is $k^2$ times less for each analyst. Now lets consider the "Fair Workload strategy" mechanism. In this mechanism instead of scaling according to the Frobenius norm of a matrix we let an optimizer choose in order to maximise the egalitarian social welfare. Now we note that if we consider the independent version of this mechanism ( in order to find error to prove the Sharing Incentive) it would simply optimize the scaling factor of the matrix for one individual to minimize their error. However since we just proved that any arbitrary scaling doesn't change the error it will effectively do nothing. Therefore all 4 versions of this mechanism have the same baseline error for the independent case.\\

The fact that scaling the entire matrix alone doesn't change the error is super helpful. Because say I have some optimal weights for the unified workload strategy $\alpha_1 W_1 \cup \alpha_2 W_2 \cup \dots \alpha_k W_k$ then multiplying them all by some factor $\beta$ doesn't change any of the errors. Therefore I might as well scale them down such that $\sum_i \alpha_i = 1$. This now bounds our problem to find the optimal set of weights such that all the weights sum to one.  \\
We also know the optimum weights for each analyst, that simply being their own workload with a weight of 1 and the others with a weight of zero. \\
Thoughts on how to solve from here \\
Goal is to maximise min-max fairness.
If every ones individual workload is the best for them and moving towards that is always better the answer is simple. use a sort of waterfilling redistribution algorithm until we hit some level of convergence but that isn't always the case. We could have a case for example where analyst 1 chooses some workload and analyst 2 chooses some other workload which happens to be more optimal for the strategy for analyst 1. An example of this is as follows. Analyst 1 chooses the all range workload. Analyst 2 chooses the workload that represents the H2 algorithm. H2 being specifically designed for that case scores better than the workload strategy.

\subsection{Defining non-triviality}
The goal of a non-triviality condition is to rule out options that involve not leveraging the joint nature of the problem. In this case a definition of non-triviality should rule out mechanisms that answer each of the query sets independently of one another. Since the definition we use for the Sharing Incentive compares any mechanism to itself it alone is not sufficient for the type of non-triviality we are looking for. It allows any mechanism that doesn't change at all when giving the group setting instead of the singular one. \\ 
We considered the idea of Pareto-optimally as a definition of non-triviality. We still get the same issue if our definition of Pareto optimality considers only the given inputs and the respective output space of the same mechanism then it still allows for Independent Mechanisms. For example consider the independent HDMM. If we assume that the optimizer for HDMM is perfect and picks the optimal strategy matrix for the given workload then the independent HDMM with respect to it's possible outputs always optimizes on the sum of the utilities across all agents. This set of query answers that optimizes on the sum of utilities must always be Pareto efficient since if there was a set of query answers that didn't reduce any utility but increased the utility for at least one person it would increase the the sum of utilities and that contradicts our perfect optimizer assumption. \\ 
Pareto-optimality seems to be a good starting point but it can't have the mechanism be compared to itself. It needs to compare the mechanism in question to some baseline that we consider to be "inefficient but reasonable". We could say that it needs to be strictly better than some baseline mechanism. That is for some naive solution any efficient solution should achieve better expected error for each analyst. 
\\ 
On some slightly good news. If you assume that there is a unique point that minimizes min max fairness and that our optimizer finds it then the strategy at that point must be Pareto optimal. Why? Well what would be required for the min-max fair point to not be pareto optimal. There must be a case where either everyone gets the same error and at least one person must get less error. If that one person was the person with maximum error already then the point we found didn't minimize min max fairness since we can minimize further by going to the Pareto-dominating point. If the person who gets less error is not the person with max error then the min-max error optimizing point is not unique since the Pareto-dominating point it has the same error for the analyst with the max error or less error. If it has the same error then it is an alternative point with the same min-max fairness value. If it has less error then either this analyst remains the analyst with the worst error in which case the new point dominates the old point in terms of min-max fairness as well or some other analyst becomes the analyst with maximum error in which case this is still a point that dominates the other in terms of min-max fairness.

\subsection{Property definitions and proofs 3/16/2020}
We would like a set of properties which when satisfied by any mechanism results in a mechanism that is "fair" within this context. We have 3 properties currently which seem to satisfy this criteria. First I'll enumerate those properties considered in the space of matrix mechanisms and show that they do not trivially satisfy each-other. That is show that no combination of the properties ensures the others. From there we can consider some techniques and how they satisfy such properties \par 

\subsubsection{Redefining Non-Interference}
Lets redefine Non-Interference. Now isntead of caring if you can reduce utility by chaning your workload we only care if you reduce other's utility to below that if you weren't there. More formally as follows. 
\begin{definition}[Non-interference]
Let $Err_i$ be the expected error of analyst $i$. 
A mechanism $\mathcal{M}$ satisfies Non-Interference if for every analyst $i$ with preference workload $W_i$  there does not exist an alternative workload $W_i'$ where $Err_i(\mathcal{M}(\epsilon, \mathcal{W})) > Err_i(\mathcal{M}(\epsilon, \mathcal{W}'))$ and for at least one other analyst $j \neq i$ $Err_j(\mathcal{M}(\epsilon, \mathcal{W} \setminus W_i)) < Err_j(\mathcal{M}(\epsilon, \mathcal{W}'))$
\end{definition}

Let's begin with the Sharing Incentive. The Sharing Incentive intuitively, as the name suggests, incentives any individual to join a group of analysts rather than answer their queries alone. If we assume privacy budget $\epsilon$ is a public good to be distributed we can give each of the $k$ analyst a fair their fair share of the privacy budget $\epsilon /k$. We then give the analyst two options. They can either use their fair share of the budget on their own using a prescribed DP mechanism in order to answer their queries or they can add their budget and queries to a collective pool in order to have all the queries of the collective answered under the collective privacy budget. The goal of the Sharing Incentive is grantee that joining the pool will result in at least as much utility for the agent as answering their queries on their own. Formally we define that as follows. We define a mechanism $\mathcal{M}$ to be a function that takes in as a parameter a privacy budget $\epsilon$ and a non-empty set of workloads and returns a strategy matrix $\mathbf{A}$ to answer the queries. Likewise we define the expected error of a mechanism to be the expected mean-squared error of the mechanism.

\begin{definition}[Sharing incentive]
Let $Err_i$ be the expected error of analyst $i$ and let $\mathcal{W}$ be the set of all analysts workloads. Let $\mathbf{W}_i$ be the workload of analyst $i$. 
% Note I need a decent way to introduce alternative workload notation
A mechanism $\mathcal{M}$ satisfies the Sharing Incentive if for every analyst $i$ the following holds. $$Err_i(\mathcal{M}(\epsilon,\mathcal{W})) \leq  Err_i(\mathcal{M}(\frac{\epsilon}{k},\{\mathbf{W}_i\}))$$
\end{definition}

We note that while Sharing Incentive is a good incentive for joining the collective group structure it does not grantee that the mechanism itself is efficient. For example consider the mechanism that simply returns an all zero matrix. Since this mechanism doesn't actually answer any of the queries we say it has infinite error. Likewise since any analyst experiences the same error under any conditions or parameters it trivially satisfies the Sharing Incentive. To that goal we consider a non-triviality constraint. Since all mechanisms considered are in the space of matrix mechanisms we consider Pareto-efficiency with respect to the matrix mechanisms (or possibly p-identity). We define pareto efficiency as follows.
\begin{definition}[Pareto-Efficiency (matrix mechanism space)]
A mechanism $\mathcal{M}(\epsilon, \mathcal{W})$ is pareto-efficient if it produces an output $\mathbf{A}$ such that there is no alternative strategy 
$\mathbf{A}' \in \mathbb{R}^{m \times n}$ such that every analyst gets at least as much utility under $\mathbf{A}'$ compared to $\mathbf{A}$ and at at least one analyst gets more utility under $ \mathbf{A}' $ compared to $\mathbf{A}$
\end{definition}

We are now going to show that the two previously defined criteria do not satisfy eachother in the space of matrix mechanisms. First we are going to show that there exists a mechanism which satisfies Pareto optimally and not the Sharing Incentive.
\begin{theorem}
Pareto optimality does not guarantee Sharing Incentive.
\end{theorem}
Consider the following mechanism which takes in a set of workloads and a privacy budget. Step 1 take the first workload and answer it's queries using the entire privacy budget under the optimal full rank strategy. Step 2 publish the results. This mechanism is Pareto-efficient because it maximizes utility for the first analyst and since the optimal strategy is unique \cite{Matrix} then any alternative workload would reduce the utility of the first agent. This mechanism may not satisfy the Sharing Incentive in cases where the second analyst has a workload that is significantly different to the first analyst. The mechanism will then optimize on the first analyst at the expense of the second.

We can similarly create a mechanism which satisfies the Sharing Incentive but is not pareto efficient.
\begin{theorem}
Sharing incentive does not guarantee pareto-optimality
\end{theorem}

Here we'll construct a mechanism which satisfies the Sharing Incentive but is not pareto efficient. In this case the mechanism splits the budget up amongst each analyst and answers the workloads independently. This is exactly the independent case so it must satisfy the Sharing Incentive however if each analyst has the same workload this is grossly inefficient since there exists a similar strategy which answers all the workloads and just uses the entire budget. 
\subsection{Achieving Pareto optimally}
Here I will go over and lightly prove two well known results about social welfare functions and Pareto optimality. 
\begin{theorem}
If a mechanism $\mathcal{M}$ maximises the utilitarian social welfare amongst all analysts it is Pareto efficient.
\end{theorem}
Lets prove this by contradiction. Assume a strategy $A$ output by mechanism $\mathcal{M}$ maximizes the utilitarian social welfare. That is $A$ maximises the total utility achieved by some agent. Likewise assume there is an alternative workload $A'$ that Pareto dominates $A$ that is all agents receive at least as much utility under $A'$ compared to $A$ and at least one agent receives strictly more utility. Since no agent loses more utility under $A'$ compared to $A$ the total welfare under $A'$ must be greater than that under $A$ which is a contradiction since $A$ should maximise the total welfare. \par 
Likewise we can prove the same with the egalitarian social welfare if that point is unique.

\begin{theorem}
If a mechanism $\mathcal{M}$ outputs a strategy $A$ that maximises the egalitarian social welfare  amongst all analysts and that strategy is a unique solution then it is Pareto efficient.
\end{theorem}

Likewise we'll prove this by contradiction. First assume that a mechanism $\mathcal{M}$ outputs a strategy $A$ that uniquely maximises the egalitarian social welfare. That is it maximises the minimum utility amongst all analysts. Let $x$ be the agent who has the minimum utility under strategy $A$. Assume that $A$ is Pareto dominated at by an alternative strategy $A'$ in this case at least one agent receives the more utility than under strategy $A$. If that agent is $x$ then there is a contradiction since that would mean that the egalitarian social welfare under $A'$ is greater than that under $A$. If the agent which receives more utility under $A'$ is not $x$ then since no other agent can lose utility this solution must have the same egalitarian social welfare as $A$. Since they both have the same social welfare then $A$ is no longer a unique maximising point of the egalitarian social welfare.

\subsubsection{Pareto Optimality in the matrix mechanism space}
It is clear when considering the space of matrix mechanisms any mechanism that we derive based off HDMM will be insufficient to achieve Pareto optimality. In order to show this we only need to show the case with one analyst who asks a degenerate set of queries who's  optimal strategy does not lie in the p-identity space. Since there exists one optimal full rank solution and it does not exist in the p-identiy space there must be a solution which pareto dominates any HDMM based solution.

\subsubsection{Pareto optimality in the p-identity space}
If we consider pareto optimality in the p-identity space then we get some conditions in which Pareto optimality may be achieved. Like previously stated any mechanism which maximises the utilitarian social welfare is Pareto optimal, the same goes for the egalitarian social welfare given that the point is a unique solution.\\
\textbf{SIDENOTE}: \\
Like how we created the fair-hdmm by changing the optimization function to the egalitarian social welfare after some scaling we can simply create a utalitarian version of hdmm by the same virtues. Since the sum of convex functions is also convex we can simply change the optimization task to maximize the sum of all agents utilities. Likewise the resulting new gradient is the sum of all the individual gradients. Since optimization on the utilitarian social welfare enforces pareto efficiency this mechanism is pareto efficient.

\subsection{Non-Interference }
Non-interference as stated above is a property of the privacy mechanism which states that no individual acting for their own good can increase their utility at the cost of others. Yikai has shown where there are cases in which lying about your workload can reduce the utility of all agents. \\
First we show that satisfying Non-Interference does not imply pareto efficiency or Sharing Incentive. We do this by giving examples of poorly designed mechanisms that don't satisfy one of the two by design but satisfy Non-Interference. Lets start with the previously discussed mechanism which doesn't answer all queries this mechanism clearly satisfies Non-Interference and the Sharing Incentive but is not pareto efficient. This gives rise to the following two theorems. 
\begin{theorem}
Non-interference does not imply pareto efficiency
\end{theorem}
\begin{theorem}
Non-interference and Sharing Incentive does not imply pareto efficiency
\end{theorem}

The second mechanism will be a slight change to the standard hdmm. In this mechanism we take in as input all the workloads of all analysts and instead of using them we just send in a random workload to HDMM. Since the actual inputs do not affect the output of the mechanism it satisfies Non-Interference but since the expected utility each time is essentially random it does not satisfy the Sharing Incentive. Therefore the following theorem holds

\begin{theorem}
Non -interference does not imply Sharing Incentive
\end{theorem}

What we've effectively learned is that we can achieve Sharing Incentive by ignoring the group structure and we can achieve Non-Interference by ignoring the input. By having a mechanism that broadly does both achieves both but cannot be Pareto efficient.

Now the question is imagine we had some magic mechanism that magically knows the analysts true intentions and therefore doesn't use the input and can simply choose from any pareto efficient point, can this mechanism satisfy the Sharing Incentive. This basically boils down to from the set of pareto-efficient solutions is there always a solution which satisfies the Sharing Incentive. In the individual case this mechanism just maximises the individual with $1/\epsilon$ of the budget.
\section{First idea}
Let current error be $U$. Let the expected error in the independent case be $\alpha$ 
The first optimization idea is as follows 
$ \max \min U- \alpha $

We then transform this into a minimization problem as follows. 

$ \min \max_i  \alpha_i - U_i , 0$


\subsection{Alternative HDMM (Name in progress)}
Consider an alternative HDMM that optimizes the following social welfare function. 
\[ \min{\{ \mathbf{A = A( \Theta)| \Theta \in \mathbb{R}^{p \times n}_+}\}} \max_{W \in \mathcal{W}}  \|\mathbf{WA^+}\|_F^2- \|\mathbf{WA_W^+}\|_F^2 -  \].

Where $ \mathcal{A_W}$ is the strategy matrix chosen by independent HDMM. The objective of this function is to specifically achieve Sharing Incentive. We note that the utility function is negative so long as any individual is getting less utility than mandated by Sharing Incentive. Therefore we note that so long as there exists a strategy matrix that satisfies Sharing Incentive given the workloads this mechanism will satisfy Sharing Incentive. 

\subsubsection{Proof of Pareto efficiency}
Assume there is a unique strategy matrix which maximises this utility function. We call this matrix $\mathbf{A}$. Assume there is an alternate strategy matrix $\mathbf{A'}$ which is Pareto dominant over $\mathbf{A}$. Since it is pareto dominant then no individual can lose utility while at least one individual sees a gain in utility. If that individual is not the worst off individual in terms of the social welfare function then $\mathbf{A}$ is not a unique optimizer.  If the individual which gains utility is thew worst off then $\mathbf{A}$ does not optimize this function therefore a contradiction. Therefore if the optimizer of this function is perfect it chooses a Pareto optimal strategy matricx.


==> Proofs.tex <==
\section{Proofs of Properties}\label{sec:proofs}
\subsection{Utilitarian Social welfare}
Here we prove that Utilitarian HDMM which vertically stacks the workload matrices is equivalent to directly optimizing on the Utilitarian social welfare objective.
\begin{theorem} \label{thrm:Utilitarian}
Optimizing on a stacked workload is equivalent to optimizing the utilitarian social welfare objective
\end{theorem}


For any $\bm{W}$ of $m$ rows, the objective function optimized on is as follows.
\[\|\mathbf{WA^+}\|_F^2 = \sum_{i=1}^m \|\bm{W}^{(i)}\bm{A^+}\|^2, \]
where $\bm{W}^{(i)}$ is the $i$th row of $\bm{W}$.
Let $\bm{W}_U$ be the vertical stack of $\bm{W} \in \cm{W}$, let $k$ be the number of workloads and $M$ be the sum of rows of each workload $m_i$, we have
\begin{align*}
    \|\bm{W}_U\bm{A^+}\|_F^2 &= \sum_{i=1}^M \|\bm{W}_U^{(i)}\bm{A^+}\|^2\\
    &=\sum_{i=1}^k\sum_{j=1}^{m_i}\|\bm{W}_i^{(j)}\bm{A^+}\|^2\\
    &=\sum_{i=1}^k\|\bm{W}_{(i)}\bm{A^+}\|^2\\
\end{align*}
which is equivalent to the Utilitarian social welfare objective.



\subsection{Proof of \cref{thrm:waterfilling}}
We will prove that the HDMM waterfilling mechanism satisfies the Sharing Incentive and Non-Interference by instead proving a stronger grantee. We will prove that increasing the number of analysts cannot decrease the utility experienced by any singular analyst. This property assures that the mechanism satisfies both properties.  \par 
Let $\bm{A}$ be the strategy matrix produced by HDMM waterfilling for $k$ analysts and $\bm{A'}$ be the strategy matrix for $(k+1)$ analysts (adding one from previous case). Each analyst has budget $\epsilon$. Each analyst's strategy matrix $\bm{A}_i$ is a submatrix of $\bm{A}$. \par 
First let us prove a few properties of HDMM waterfilling. 
\begin{lemma}
The introduction of an additional analyst to the HDMM waterfilling mechanism can only increase the sensitivity of the final strategy matrix by 1.
\end{lemma}

We first note that the strategy matrix produced by HDMM waterfilling in the single analyst case is exactly the same strategy used by the standard HDMM mechanism. Since this strategy is part of the p-identity space it all of it's columns have norm 1. If we add an additional analyst for each of the new analysts queries they may either add their query to an existing bucket or create a new bucket for their query. For each query $v$ if that query were to belong to an existing bucket with representative query $e$ and weight $w$ then $v$ would be added to the bucket and the new weight would be $\norm{v} + w$. As such the bucket would be represented in the final matrix as $(\norm{v} + w)e$. Since $v$ belongs to the bucket it is by definition equal to $\norm{v}e$. Therefore the final represented query in the matrix is equivalent to the existing query plus the new query being added into the bucket $(\norm{v} + w)e = \norm{v}e +we$. Therefore the column norm of the matrix can be raised by at most $\norm{v}$. Likewise if the query $v$ belongs in it's own bucket is is merely added to the final strategy matrix as is therefore only increasing the column norm of the strategy matrix by a maximum of $\norm{v}$. However since all the queries being added to the final strategy matrix are done by either appending or addition the overall increase to the column norm of the final matrix is equal to the column norm of the strategy matrix chosen by the additional analyst. As stated before this matrix has a column norm of 1. \par 

% alternative shorter version
We first note that the strategy matrix produced by HDMM waterfilling in the single analyst case is exactly the same strategy used by the standard HDMM mechanism. Since this strategy is part of the p-identity space it all of it's columns have norm 1. If we add an additional analyst for each of the new analysts queries they may either add their query to an existing bucket or create a new bucket for their query. If the query belongs in it's own bucket then the query is simply appended to the final workload. If the query belongs into an existing bucket then that query is simply added to the existing representative query of that bucket. Since all of queries introduced by the additional analyst are added to the matrix by either appending or adding to existing queries the final increase to the sensitivity of the strategy matrix is equal to the sensitivity of the strategy matrix chosen by the additional analyst.


Likewise we can represent the unified strategy matrix under HDMM waterfilling as a matrix of representative queries $\bm{A}$ multiplied by a scaling matrix of weights $\bm{D}$. Let $\bm{A}$ and $\bm{D}$ be the unified strategy and weight matrix under HDMM waterfilling with all $k$ analysts.Let $\bm{A'}$ and $\bm{D'}$ be the unified strategy and weight matrix under HDMM waterfilling with $k-1$ analysts 
As stated before we have $\|\bm{DA}\|_1 =\sum_i\|\bm{A}_i\|_1 = k$. Similarly,
$\|\bm{D'A'}\|_1 = k-1$. Let $\bm{W}$ be the workload of any analyst.  Then the error experienced by any particular analyst is as follows.
\begin{align*}
Err(\mathbf{W},\mathbf{A}) &=\frac{2}{k^2\epsilon^2}\|\bm{DA}\|_1^2 \|\bm{W(DA)^+}\|^2_F\\ &= \frac{2}{k^2\epsilon}k^2\|\bm{WA^+D^+}\|^2_F\\
&=\frac{2}{\epsilon^2}\|\bm{WA^+D^+}\|^2_F\\
&= \frac{2}{\epsilon^2(k-1)^2}(k-1)^2\|\bm{W}\bm{A^+D^+}\|^2_F\\
&\leq \frac{2}{\epsilon^2(k-1)^2}\|\bm{A'}\|_1\|\bm{W}\bm{A'^+D'^+}\|^2_F.\\
&=Err(\mathbf{W},\mathbf{A'}).
\end{align*}
Since $\bm{A'}$ is a submatrix of of $\bm{A}$ then every row of $\bm{D'A'}$ is either in $\bm{DA}$ or a portion (multiple with positive ratio less than 1) of a row of $\bm{DA}$. Therefore   $\|\bm{W}\bm{A'^+D'^+}\|^2_F \leq \|\bm{W}\bm{A^+D^+}\|^2_F$ 
\dap{TODO: confirm this?}


\subsection{Proof of \cref{thrm:waterfilling} generic version}
We will prove that waterfilling mechanisms satisfies the Sharing Incentive and Non-Interference by instead proving a stronger grantee. We will prove that increasing the number of analysts cannot decrease the utility experienced by any singular analyst. This property assures that the mechanism satisfies both properties.  \par 
Let $\bm{A}$ be the strategy queries produced by a waterfilling mechanism for $k$ analysts and $\bm{A'}$ be the strategy queries for $(k+1)$ analysts (adding one from previous case). The $i$th analyst has budget $s_i\epsilon$. Each analyst's strategy queries $\bm{A}_i$ is a subset of $\bm{A}$. \par 
First let us prove a few properties of HDMM waterfilling. 
\begin{lemma}
The introduction of an additional analyst with weight $s'$ to the collective of a waterfilling mechanism can only increase the sensitivity of the query set by $s'$.
\end{lemma}

\begin{proof}
When a new analyst is added to the collective for each of their queries they have two options they may either create a new bucket or add their query to an existing bucket. If they add a new bucket that query becomes part of the final strategy query set adding it's sensitivity to the overall sensitivity. If they add their query to an existing bucket  the weight of that query increases by the weight of that query, therefore increasing the overall utility by the weight of that query. Since the weight of all of an analysts queries must equal their overall weight the increase in sensitivity is equal to the overall weight of the analyst.
\end{proof}

We note that since each analyst is entitled to $s_i\epsilon$ of the budget and the sensitivity of the strategy query set is equal to the sum of each analysts weights that the scale of the noise used to answer the query set is the same regardless of the number of analysts in the collective. The scale of the noise added to the query set is as follows. 
$$ \frac{\norm{A}_1}{\epsilon} = \frac{\sum_{i=0}^k s_i}{\sum_{i=0}^k s_i \epsilon} = \frac{1}{\epsilon}$$

We now consider two different perspectives when an additional analyst, Bob, is added to the collective. We first consider the case of an analyst who is already in the collective, Alice,  and how their utility is affected by an additional analyst joining. We then consider the case of the analyst joining the collective and how their utility changes as they join the collective.
\par
Consider Alice, an analyst already in the collective. If the new analyst being added shares no queries with Alice then her queries remain unchanged and the noise being added stays the same ensuring that her query answers remain utility neutral. If Bob shares queries with Alice then the weights of Alice's queries will increase. This reduces the the amount which Alice's queries need to be re-scaled to reconstruct her original strategy queries therefore reducing her error. Since adding Bob to the collective is either utility neutral or positive for Alice the mechanism satisfies Non-Interference. \ par 
Likewise consider Bob an analyst to be added to the collective. From Bob's perspective adding Bob to the existing collective is equivalent to adding all the members of the existing collective to Bobs collective (of just himself). Just like Alice adding any analysts to Bobs collective is either utility neutral or positive. Since Bobs collective of just himself is indeed the independent case and if being added to the collection is either utility neutral or positive then the mechanism satisfies the Sharing Incentive.

==> Response_letter.tex <==

\begin{center}
    \textbf{Revision Letter: Paper $\# 726$ }
\end{center}

We would like to thank the reviewers for their detailed and insightful comments which have been immensely helpful in the revision process. We have significantly revised our paper in terms of completeness and readability. We have highlighted (in blue) all new and edited text in the main paper for ease of reference. The following section outlines the changes to the paper.

\myparagraph{Meta Review}
\begin{itemize}
    \item\textbf{Major point 1:}  \textit{Better discussion of tradeoff between privacy and accuracy (R4D1)}
    \\ \\
    We have added a new section \cref{sec: Tradeoffs} titled ``Tradeoffs Between Desiderata and Accuracy'' where we discuss how satisfying Sharing Incentive and Non-interference may necessitate lower accuracy; but satisfying adaptivity does not. We also add a discussion in \cref{sec:prac_results} where we show that a mechanism which satisfies all three desiderata, such as the Waterfilling Mechanism, does not outperform a mechanism which is only adaptive such as the Utilitarian mechanism but does outperform a mechanism which satisfies both the Sharing Incentive and Non-interference such as the Identity mechanism.\\
    
    \item \textbf{Major point 2: } \textit{Consider alternative approach based on matrix mechanism (R5D1)}
    \\ \\ 
    Reviewer 5's suggestion of an alternative mechanism which incorporates previous knowledge is very interesting as it is it is a simple and intuitive mechanism for the multi analyst problem. However, to the best of our knowledge, there is no state of the art way to incorporate prior knowledge into the matrix mechanism optimization step. From the reviewers description, we were able to come up with two different mechanisms - one that did not satisfy the desiderata and one that did satisfy all the desiderata but performs worse than identity. The first mechanism is as follows.
    \begin{itemize}
        \item Order the agents from greatest to least $\epsilon_i$
        \item For each agent i:
        \begin{itemize}
            \item If $W_i$ inferable from $\{W_j | j < i\}$, use inference for $W_i$ 
            \item Else, disregard above and run Matrix on $W_i$ with $\epsilon_i$
        \end{itemize}
    \end{itemize}
    Consider a case with only two analysts, Alice and Bob. In this case, Alice and Bob have different queries. Each analyst has exactly half the privacy budget. Alice asks the Identity workload and Bob asks the Total workload. First Alice's queries are answered independently. Then, the mechanism realizes that Bob's queries can be reconstructed using Alice's queries and does so. Now Bob's queries are reconstructed using $n$ noisy counts when it would have been answered directly if he was the only analyst. In this case even if Alice's queries were answered using the entire privacy budget, Bob would have preferred to answer his query directly using his half of the privacy budget resulting in a violation of the Sharing Incentive.
    
    The second Mechanism is as follows.
    \begin{itemize}
        \item Order the agents from greatest to least $\epsilon_i$
        \item For each agent i:
        \begin{itemize}
            \item If $W_i = W_j$ for j before i
            \item Else, disregard above and run Matrix on $W_i$ with $\epsilon_i$
        \end{itemize}
    \end{itemize}
    This mechanism is generally inefficient as it may lead to a waste of privacy budget. Consider the case where there are two analysts Alice and Bob. Alice and Bob both have the exact same queries. The mechanism will first answer the queries using Alice's budget. Then when it is Bob's turn his queries will be answered with a reuse of Alice's query answers. However now Bob's privacy budget is never used. At least with the Independent Mechanism both analysts will be presented with two different answers to the same query using different privacy budgets which can then be combined in post processing.
    
    To the best of our knowledge there is no  variant of the matrix mechanism which incorporates prior knowledge into it's optimization task. We consider this to be a significant open problem worthy of a paper in its own right. We have added a discussion of remaining technical challenges including incorporating prior knowledge and adapting the problem to the online setting in \cref{sec:Future_work}. We consider the Waterfilling mechanism to be a simple solution that satisfies all the desiderata while remaining relatively efficient. Improving the Waterfilling Mechanism (or other mechanisms) to properly incorporate prior knowledge is an interesting avenue for future research.\\
    
    
    \item \textbf{Minor point 1:}\textit{Discuss the impact of analysts arriving and departing (R4D2)} \\ \\
    In the static setting, the collective of analysts where analysts may join and leave as they please is used as a tool to illustrate the desiderata and what should be expected of any multi-analyst DP mechanism. However in an online setting where analysts may ask queries adaptively and may join the collective dynamically, joining the collective may have significant impact on the other analysts. As such, we have discussed the remaining technical challenges and future work in \cref{sec:Future_work}. Here we discuss remaining challenges such as distributing budget in an online manner and incorporating prior knowledge into the matrix mechanism.\\
    
    \item \textbf{Minor point 2:}\textit{Clarifications on methods and experiments (R4D3, R5D2, R6D3, R6W2, R6W3)}\\ \\
    We have reordered and reworked \cref{sec:Experiments} in order to make it more clear. The new structure goes over the setup for each experiment individually then goes on to give the results for each experiment individually. We hope that this structure is clearer and easier to understand. Likewise we have included additional discussions on how budget is divided in our experiments in  \cref{sec:Experiments_WorkloadsAndDatasets}. We have also added additional discussions on higher values of $\tau$ in \cref{Sec:Experiments_Tolerance_setup} stating that the trend shown in the figures holds for higher values of $\tau$ but have been omitted from figures for clarity.
\end{itemize}
\myparagraph{Review \# 4}
\begin{itemize}
    \item \textbf{D1, W1:} \textit{ The trade-off between privacy (in terms of the three desiderata) and utility should be further explained and justified.} \\ \\
    We have added a discussion of the trade offs between our desiderata and accuracy in \cref{sec: Tradeoffs}. Likewise we have analyzed what role these trade-offs play in \cref{sec:Experiments}. It is important to note that a mechanism does suffer some accuracy loss in order to satisfy both Sharing Incentive and Non-interference. Unlike the other two desiderata adaptivity is not orthogonal to accuracy. It is expected that a mechanism which is able to adapt to different workloads would perform better on average than a mechanism which statically uses the same strategy regardless of the inputs. This can be seen through our results as the Waterfilling mechanism performs more poorly than the Utilitarian Mechanism which only satisfies adaptivity but performs better than identity which satisfies both the Sharing Incentive and Non-interference but not adaptivity. We have edited the results discussion to further emphasise this relationship.\\
    
    \item \textbf{D2, W3:} \textit{The proposed framework only applies to a static setting.}\\ \\
    In our work we focus mainly on data independent mechanisms which restricts our problem to the offline setting as most state of the art mechanisms in the online setting are data dependent. Likewise it is unclear how our desiderata could be expanded to the online setting where analysts can dynamically join the collective. We agree that allowing analysts to dynamically join the collective is an interesting avenue for future work. \\
    
    \item \textbf{D3, W2:}\textit{ Some technical details of the DP mechanisms need further clarification.}\\ \\ We have added a statement in what is now \cref{sec:Experiments} stating that in our experiments we give all analysts an equal share of the privacy budget as well as a statement giving the total privacy budget used. In addition we clarify in what is now \cref{Sec:Experiments_Tolerance_setup} that we have experimented with a larger range of $\tau$ however have chosen to omit it from the figures for clarity. Likewise we have reworked \cref{sec:waterfilling} in order to better explain the Waterfilling Mechanism. Similarly to how we present the desiderata \cref{sec:waterfilling} now begins with a simplified example with additional details afterwards. We hope these changes further clarify the intuition behind the Waterfilling Mechanism.
\end{itemize}

\myparagraph{Review \# 5}
\begin{itemize}
    \item \textbf{D1, W1:}  \textit{The paper overlooks a simple approach to satisfy the three desiderata considered.}\\ \\
    We consider the approach brought up by the reviewer to be very interesting. From the reviewers rubric we were able to make two different mechanisms one of which did not satisfy the desiderata and the other which did not outperform the baseline. We go into more detail in the meta review section. We thank the reviewer for their suggestion and will consider the application of prior knowledge when improving the Waterfilling Mechanism. \\
    
    \item \textbf{D2: W2} \textit{The analysis on the Weighted Utilitarian Mechanism is incomplete.}\\ \\
    We have added additional statements in what is now \cref{sec:Experiments_WorkloadsAndDatasets} which states that the Weighted Utilitarian Mechanism does not satisfy Non-interference as seen in experiments. We also conjecture that the Weighted Utilitarian Mechanism satisfies the Sharing Incentive as it is directly optimizing to do so and we have not been able to construct an instance where the Weighted Utilitarian Mechanism fails to satisfy the Sharing Incentive.
\end{itemize}

\myparagraph{Review \# 6}
\begin{itemize}
    \item \textbf{W1:}\textit{Throughout the paper, the authors use terms and concepts (that may perhaps be familiar to readers familiar with differential privacy) without defining them or even providing an intuition. For example, Definition 2 introduces the symbol A without context; It is later referenced as a strategy workload without further context. At least a little intuition for how A is selected would be helpful. Similarly, multiple norms are used. It is *maybe* safe to assume that the reader understands the term "L2-norm", but it would be helpful to define e.g., the frobenius norm. Likewise, $f_B(e)$ in S4.3 is never defined.}\\ \\
    We have reworked the proofs in  \cref{sec:waterfilling} in order to avoid using previously undefined functions like $f_B(e)$. Likewise we have reworked \cref{sec:background} in order to better define strategy workloads before using them in notation.  \\
    \item \textbf{W2:} \textit{S4 does a fantastic job of exploring the design space at both an abstract design space level, as well as providing concrete examples of specific algorithms in the space. However, it's a little unclear the role that these algorithms serve. Are the supposed to be examples of prior work in the space? Are they simply illustrative of potential solutions in the space? Are they novel contributions? If the former, direct citations in S4 would be helpful. If the second, then the (unjustified) implication in the experimental results is that the examples are representative of their class. }\\  \\
    In order to clarify the purpose of each of the algorithms presented we have reworked the algorithms section and split it into two distinct parts. In the first part we discuss the classes of mechanism (now renamed to design paradigms). This has been done to emphasise that these are merely the design paradigms we followed when designing mechanisms and that each has clear advantages and disadvantages. We note that these paradigms are not exhaustive of all the possible mechanisms in this space. The second part contains the algorithms themselves which we have further divided into 3 parts. The first part discusses existing mechanisms in this space and contains the independent mechanism and Identity mechanism. The second part contains mechanisms that have been lightly adapted to fit in this problem setting. This section contains the Utilitarian mechanism and Weighted Utilitarian mechanism as they are adaptations of HDMM. The final section contains the main contribution in the Waterfilling Mechanism. \\
    \item \textbf{W3:} \textit{What appears to be the paper's main contribution: the Waterfilling Mechanism, is presented without much design justification. It clearly is an example of a select first mechanism, but the actual mechanism is only explained superficially in S4.3. The algorithm itself is full of what seem like arbitrary constants that really need to be explained. }\\ \\ We have reworked \cref{sec:waterfilling}. It now begins with a simplified example of the Waterfilling Mechanism as shown in \cref{fig:waterfill_animation} and then introduces and justifies the additional steps done in the full Waterfilling Mechanism. This includes some new text introducing and justifying the additional parameter $\tau$. 
    \\
    \item \textbf{D1: } \textit{ Lemma 3 seems to be trivially true, since the L1 norm of every column is 1. Am I missing something? (If so, it might help a typical reader to provide an intuition for what is not obvious here.}\\ \\
    Since all the column norms are 1 lemma 3 is trivially true. We chose to include the proof for lemma 3 in the text in order to be thorough as other parts of the proof depend on it. We also include the proof in order to justify why we require the constraint that all column norms are 1 in the selection step. \\
    \item \textbf{D2: }\textit{On page 8, left column: Why introduce a new variable x? k seems like it would fit here.}\\ Here we introduce a new variable in order to demonstrate that this holds for any arbitrary number of analysts not only all the analysts $k$. We have renamed the variable to $z$ since we had used $x$ to denote the data vector previously.
    \item \textbf{D3:} \textit{Why only one experimental workload?}\\ \\ In our experiments we use a randomized process in order to generate multiple instances of the problem where there are a random number of analysts and each analyst has a randomized workload. The process used is discussed in \cref{sec:prac_setup}. We have reorganized the experiments section to make it more clear how the problem instances are created for each set of experiments. We have created two separate subsections containing the methods used in the experiments as well as results of said experiments respectively. We hope that this reorganization makes it more clear as to how the experiments were conducted.
\end{itemize}

\myparagraph{Additional Changes}
We thank all the reviewers for acknowledging and noting some typos and grammatical errors in the paper. Changes have been made fixing such errors and have been appropriately highlighted.


==> algos_table.tex <==
%testing box
% Spanning graphic for mechanism classes without desiderata
\begin{figure*}[t]
\resizebox{0.75\textwidth}{!}{%
	\centering
	\begin{subfigure}[b]{0.35\textwidth}
		\includegraphics[width=1\textwidth]{fig/Independentanimation.pdf}
		
		\caption{Independent}\label{fig:independent}
	\end{subfigure}
	\begin{subfigure}[b]{0.35\textwidth}
		\includegraphics[width=1\textwidth]{fig/Workload_agnostic_animation.pdf}
		
		\caption{Workload Agnostic}\label{fig:agnostic}
	\end{subfigure}
}
\resizebox{0.75\textwidth}{!}{%
    \begin{subfigure}[b]{0.35\textwidth}
		\includegraphics[width=1\textwidth]{fig/Collect_first_animation.pdf}
		
		\caption{Collect First}\label{fig:collect}
	\end{subfigure}
	\begin{subfigure}[b]{0.35\textwidth}
		\includegraphics[width=1\textwidth]{fig/Select_first_mechanism.pdf}
		
		\caption{Select First}\label{fig:select}
	\end{subfigure}
}
\caption{Mechanism Classes for Multi-Analyst DP Query Answering}
\label{fig:algos}
\end{figure*}

% single column desiderata
\begin{table}[t]
\caption{Desiderata satisfied by algorithms}
\begin{tabularx}{\columnwidth}{|l|X|X|X|}
    \hline
     \diagbox[width=0.36\hsize]{\textbf{Mechanism}}{\textbf{Desiderata}} &  Sharing\newline Incentive  & Non-interference & Adaptivity\\
    \hline
    Independent  & \cmark   & \cmark & \cmark  \\
    \hline
    Identity  & \cmark & \cmark & \xmark\\
    \hline
    Utilitarian & \xmark & \xmark & \cmark\\
    \hline
    Weighted Utilitarian  & \qmark  & \xmark & \cmark \\
    \hline
    0-Waterfilling  & \cmark & \cmark & \cmark \\
    \hline
\end{tabularx}
\label{tab:algos}
\end{table}

% Original spanning graphic with mechanism classes and desiderata
\begin{comment}
\begin{table*}[t]
\caption{Desiderata satisfied by algorithms}
\resizebox{\linewidth}{!}{%
\begin{tabular}{|c|c|c|c|}
    \cline{2-4}
     \multicolumn{1}{c|}{}  & {\footnotesize Sharing Incentive}  & {\footnotesize Non-interference} & {\footnotesize Adaptivity}\\
    \hline
     { \footnotesize Independent Mechanism}  &   &  &  \\
     \includegraphics[width = 0.25 \linewidth]{fig/Independentanimation.pdf}  & \cmark   & \cmark & \cmark\\ 
    \hline
    {\footnotesize Workload Agnostic Mechanism} &  &  & \\
    \includegraphics[width = 0.25 \linewidth]{fig/Workload_agnostic_animation.pdf} & \cmark & \cmark & \xmark\\
    \hline
    {\footnotesize Collect First Mechanism} & & &\\
    \includegraphics[width = 0.25 \linewidth]{fig/Collect_first_animation.pdf} & \xmark & \xmark & \cmark\\
    \hline
    {\footnotesize Select First Mechanism}  & & & \\
    \includegraphics[width = 0.25 \linewidth]{fig/Select_first_mechanism.pdf} & \cmark & \cmark & \cmark\\ 
    \hline
\end{tabular}}
\label{tab:algos}
\end{table*}
\end{comment}


\begin{comment}
\begin{table*}[th]
\caption{Desiderata satisfied by algorithms}
%\resizebox{\linewidth}{!}{%
\begin{tabular}{|c|c|c|c|}
    \cline{2-4}
     \multicolumn{1}{c|}{}  & Sharing Incentive  & Non-interference & Adaptivity\\
    \hline
    Independent Mechanism  & \cmark   & \cmark & \cmark  \\
    \hline
    Identity Mechanism  & \cmark & \cmark & \xmark\\
    \hline
    Utilitarian Mechanism & \xmark & \xmark & \cmark\\
    \hline
    Weighted Utilitarian Mechanism  & \qmark  & \xmark & \cmark \\
    \hline
    Waterfilling Mechanism  & \cmark & \cmark & \cmark \\
    \hline
\end{tabular}%}
\label{tab:algos}
\end{table*}
\end{comment}



==> pastebin.tex <==
\begin{figure*}[t]
\resizebox{\textwidth}{!}{%
	\centering
	\begin{subfigure}[b]{0.315\linewidth}
		\includegraphics[width=1\textwidth]{fig/prac_total_errors.pdf}
		\caption{Total errors (log scale)}
		\label{fig:prac_total}
	\end{subfigure}
	\begin{subfigure}[b]{0.32\linewidth}
		\includegraphics[width=1\textwidth]{fig/prac_max_ratio_errors.pdf}
		\caption{Max ratio errors}
		\label{fig:prac_ratio}
	\end{subfigure}
	\begin{subfigure}[b]{0.31\linewidth}
		\includegraphics[width=1\textwidth]{fig/prac_inters.pdf}
		\caption{Empirical interference}
        \label{fig:prac_inter}
    \end{subfigure}%
}
\caption{Practical setting}
\label{fig:prac}
\end{figure*}
\begin{figure*}[t]
\resizebox{\textwidth}{!}{%
	\centering
	\begin{subfigure}[b]{0.315\linewidth}
		\includegraphics[width=1\textwidth]{fig/marginal_total_errors.pdf}
		\caption{Total errors (log scale)}
		\label{fig:marginal_total}
	\end{subfigure}
	\begin{subfigure}[b]{0.32\linewidth}
		\includegraphics[width=1\textwidth]{fig/marginal_max_ratio_errors.pdf}
		\caption{Max ratio errors}
		\label{fig:marginal_ratio}
	\end{subfigure}
	\begin{subfigure}[b]{0.31\linewidth}
		\includegraphics[width=1\textwidth]{fig/marginal_inters.pdf}
		\caption{Empirical interference}
        \label{fig:marginal_inter}
    \end{subfigure}%
}
\caption{Marginal Workloads}
\label{fig:marginal}
\end{figure*}
\begin{figure*}[t]
\resizebox{\textwidth}{!}{%
	\centering
	\begin{subfigure}[b]{0.33\linewidth}
		\includegraphics[width=1\textwidth]{fig/data_total_errors.pdf}
		\caption{Total errors (log scale)}
		\label{fig:data_total}
	\end{subfigure}
	\begin{subfigure}[b]{0.255\linewidth}
		\includegraphics[width=1\textwidth]{fig/data_total_errors_2.pdf}
		\caption{Total errors (Zoomed in)}
		\label{fig:data_total_zoom}
	\end{subfigure}
	\begin{subfigure}[b]{0.198\linewidth}
		\includegraphics[width=1\textwidth]{fig/data_max_ratio_errors.pdf}
		\caption{Max ratio errors}
		\label{fig:data_ratio}
	\end{subfigure}
	\begin{subfigure}[b]{0.202\linewidth}
		\includegraphics[width=1\textwidth]{fig/data_inters.pdf}
		\caption{Interference}
        \label{fig:data_inter}
    \end{subfigure}%
}
\caption{Data-dependent Nonlinear Workloads}
\label{fig:data}
\end{figure*}



 %old introduction paragraph.
 
 More specifically we consider the problem where a large organization (known as the data curator) has a dataset in which multiple analysts or stakeholders are interested. Each analyst may represent an individual with specific queries they want answered or other organizations with some kind of vested interest in the dataset in question. Each of these analysts represent their interest in the dataset as a set of queries which the analyst want answered. The data curator then answers the queries of all analysts in some differentially private manner using a fixed privacy budget $\epsilon$. Through in reality the entirety of the privacy budget belongs to the data curator one can imagine the privacy budget as a finite resource where each analyst is entitled to some fraction of it. If the privacy budget is a resource to be allocated this raises the question. \textit{``How should one design a privacy mechanism when multiple analysts may be in competition over the limited privacy budget''}. \par
 
 
 
 
 %old introduction in its entirety 
 Large data collecting organizations, like Facebook and Google, and federal institutions, like The U.S. Census Bureau and Medicare, often release summary statistics about individuals and populations. These data products are incredibly useful tools for multiple resource allocation, policy-making and scientific endeavors. The US census alone informs agencies across the country as to how to apportion resources.  Decisions like congressional seat apportionment, school funding and emergency response plans all depend on census data \cite{Census_uses}. Google's releases of search trends or map data inform many companies' advertisement and logistics strategies \cite{Gmaps_data}. Likewise Facebook's trove of user interaction data was found to be valuable in studying the impact of social media on elections and democracy \cite{FacebookSocialScienceOneData}. 


While these data releases are very useful, they have the potential to reveal sensitive information about individuals, especially through the analysis of multiple such datasets \cite{haney2017,machanavajjhala_privacy_on_the_map,vaidya_2013}. As a result, Differential Privacy (DP) \cite{dwork2014:textbook,DiffPriv} has arisen as the gold standard of privacy protection through the addition of randomized noise.
However, due the fundamental law of information recovery \cite{dinur_nissim_2003},  making an unbounded number of releases from a dataset (even if each release were differentially private) will eventually allow an attacker to accurately reconstruct the underlying dataset. Because of this, data curators must bound the amount of information released using a parameter known as the privacy loss budget $\epsilon$. Traditional privacy mechanisms are generally focused on minimizing the overall error induced by differential privacy, where error trades off with $\epsilon$. \par 

Almost all of the work in differential privacy up until now has focused (often implicitly) on the single analyst case. In this case a single analyst specifies one or more queries or tasks that are answered under the same privacy loss budget such that the overall error is minimized. However, in the real world there are often multiple analysts or stakeholders interested in a particular dataset, and the privacy loss budget must apply across the release of answers to the queries of all of the analysts. While it is well known how to answer multiple queries or generate synthetic data under differential privacy with limited privacy budget \cite{Xu2013,Matrix10,HDMM,AHP,Chen13:recursive,Ding2011,Hay2010,Li2014,Narayan,Hb,Acs2012,torkzadehmahani2020dpcgan,PrivBays} we know of no differentially private mechanisms designed with the interests of multiple analysts in mind. %While this is beneficial when there is a single dataset for a single use this is a liability when the dataset has multiple uses.

One straightforward adaptation to the multi-analyst case is to simply aggregate the queries of all analysts into a single workload for an existing privacy mechanism. Such a mechanism then optimizes for total error and is agnostic to as to which queries belong to which analysts. Such an approach may arbitrarily exhaust more privacy budget on the queries of one agent over another, leaving some analysts with more accurate results than others. In other words, there is the potential for the queries of one analyst to \textit{interfere} with the quality of the results for another analyst. \par

Another approach is to partition each agent and give them each their own fraction of the total privacy budget to use. While this prevents the aforementioned kind of interference, it can result in a substantial overall degradation in performance when there is overlap between analyst queries. This overlap can be explicit when different analysts ask the same queries or implicit when different analysts ask related queries that can be more efficiently answered jointly than by simply answering each independently. \par

%This leaves an issue for organizations with large datasets that have multiple uses. Under existing mechanisms they may either optimize their differentially private release mechanism for a single use and abandon analysts interested in other tasks or they may create a general use differentially private release and risk wasting large portions of the privacy budget.\par

We are interested in designing effective shared systems for multi-analyst differentially private data release that achieves the best of both of these aforementioned ideas: (1) providing guarantees to individual analysts and (2) ensuring good overall performance. We call this the multi-analyst differentially private data release problem.

\noindent\textbf{Overview of approach and contributions.} Our work introduces and investigates the multi-analyst differentially private data release problem.In this problem a data curator has a dataset in which multiple analysts are interested in. Each analyst asks the data curator a set of queries to be answered in a differentially private manner. The data curator then answers all of the queries using a fixed privacy loss budget and releases the answer to all queries to each analyst. In this context we ask the question \textit{``How should one design a privacy mechanism when multiple analysts may be in competition over the limited privacy budget''}. \par
We describe three minimum desiderata which we argue that any mechanism in this setting should satisfy. These require that if an analyst was given a choice to either join a group of analysts and answer their queries together or to have their queries answered independently, with their share of the privacy budget, an analyst should always weakly prefer to join the group. We experimentally show that existing mechanisms for answering multiple queries such as HDMM \cite{HDMM} do not satisfy these properties in practical settings. We then introduce an adaptation of the existing Select Measure Reconstruct paradigm designed for the multi-analyst setting.

We show that existing mechanisms applied with no changes either do not satisfy these properties or are prone to high amounts of error. We then design and test mechanisms designed to satisfy these properties while remaining efficient.

Our main contributions in this work are as follows.
\begin{itemize}
    \item We study (for the first time)  differentially private query answering across multiple analysts. We consider a realistic setting where multiple analysts pose query workloads and the data owner makes a single private release to answer all analyst queries. 
    \item We define three minimum desiderata that that we will argue any differentially private mechanism should satisfy in a multi-agent setting -- Sharing Incentive, Non-Interference and Adaptivity.
    \item We show empirically that existing mechanisms for answering large sets of queries violate at least one of the desiderata described.
    \item We introduce variants of the existing Select Measure Reconstruct paradigm which are designed to utilize the group structure of the problem and satisfy the given desiderata in practice.   
    \item We introduce mechanisms within the adapted Select Measure Reconstruct paradigm  which provably satisfy all of the desiderata while maintaining efficiency.
    \item We show through experiments that the mechanisms which utilize the adapted Select Measure Reconstruct paradigm satisfy all the desiderata given while still remaining efficient with respect to total error.
\end{itemize}



\noindent\textbf{Organization:} In the next section we describe the relevant background information such as the definitions of differential privacy and matrix mechanisms. In section \cref{sec:background} we briefly discuss differential privacy and other required background information. In \cref{sec:ProbDef} we formally define the multi-analyst differentially private data release problem as well as some notation. In \cref{sec:desiderata} we describe the desiderata that we believe any mechanism designed for multi-analyst differential privacy should satisfy. In \cref{sec:Algorithms} we describe how existing mechanisms can be used in this setting as well as introduce new mechanisms designed for this setting. In \cref{sec:Experiments} we then test these mechanisms in both practical settings as well as pathological cases designed to violate the desiderata.



% attempted rewrite of the proofs 

\begin{theorem} \label{thrm:waterfilling}
Adding an analyst to the collective in the Waterfilling Mechanism cannot increase the expected error of any analyst.
\end{theorem}
\begin{proof}
Let $\bm{A}$ be the strategy queries produced by a Waterfilling Mechanism for $k-1$ analysts and $\bm{A'}$ be the strategy queries for $k$ analysts (adding one from previous case). The $i$th analyst is entitled to $s_i\epsilon$ of the budget. First let us prove a few properties of the Waterfilling Mechanism.
\begin{lemma}
\label{Lemma:sensitivity}
The introduction of an additional analyst with weight $s_i$ to the collective of a waterfilling mechanism can only increase the sensitivity of the query set by $s_i$, written formally in Equation~\ref{eq:wf_sensitivity}.
\begin{equation}
    \norm{\bm{A'}}_1 =  \norm{\bm{A}}_1 +s_i
\label{eq:wf_sensitivity}
\end{equation} 
\end{lemma}

When a new analyst is added to the collective, for each of their queries, either the mechanism creates a new bucket or the query is added to an existing bucket. If the former, that query becomes a representative and thus is an explicit part of the final strategy query set, adding exactly its sensitivity to the overall sensitivity. If the latter, then the weight of the corresponding bucket increases by the weight of the query, therefore increasing the overall sensitivity by the weight of that query. Since the weight of all of an analysts' queries must equal their overall weight the increase in sensitivity is equal to the overall weight of the analyst, which establishes Equation~\ref{eq:wf_sensitivity}.

We note that since the ith analyst is entitled to $s_i\epsilon$ of the budget and the sensitivity of the strategy query set is equal to the sum of each analysts' weights that the scale of the noise used to answer the query set is the same regardless of the number of analysts in the collective.Let $x$ be any arbitrary number of analysts The scale of the noise added to each query in the set is as follows. 
\begin{equation}
    \frac{\norm{\bm{A}}_1}{\epsilon} = \frac{\sum_{i=1}^x s_i}{\sum_{i=1}^x s_i \epsilon} = \frac{1}{\epsilon}
\end{equation}

We now consider two different perspectives when an additional analyst is added to the collective. We first consider the case of an analyst who is already in the collective, Alice,  and how their utility is affected by an additional analyst joining. We then consider the case of the analyst joining the collective, Bob,  and how their utility changes as they join the collective.
\par
Consider Alice, an analyst already in the collective. If the new analyst being added shares no queries with Alice then her queries remain unchanged and the noise being added stays the same ensuring that her query answers remain utility neutral. If Bob shares queries with Alice then the weights of Alice's queries will increase. This reduces the the amount which Alice's queries need to be re-scaled to reconstruct her original strategy queries therefore reducing her expected error. Therefore adding Bob to the collective can only either be error neutral or negative for Alice. \par 

Likewise consider Bob an analyst to be added to the collective. From Bob's perspective adding Bob to the existing collective is equivalent to adding all the members of the existing collective to a collective consisting of only Bob. Just like Alice adding any analysts to Bobs collective is either utility neutral or positive. Since adding an additional analyst is error neutral or negative for both Alice and Bob then no analyst can see an increase in error from an additional analyst joining the collective.
\end{proof}

Since an analyst joining the collective can not increase the error for any analyst no analyst will see an increase in error as they go from the independent case to part of the collective. Therefore any waterfilling mechanism satisfies the Sharing Incentive. 
\begin{corollary}
Any waterfilling mechanism satisfies the Sharing Incentive
\end{corollary}
Likewise due to \cref{thrm:waterfilling} no analyst joining the collective can increase the error of any analysts in the collective. Therefore the waterfilling mechanism satisfies Non-Interference. 

\begin{corollary}
Any waterfilling mechanism satisfies Non-Interference.
\end{corollary}

In practice we use HDMM~\cite{HDMM} as the selection step for this mechanism. When using matrix mechanisms or variants thereof for selection in the Waterfilling Mechanism, in addition to ensuring that each strategy matrix has sensitivity 1, each column of the strategy matrix should also have norm 1. In our experiments this is done by using HDMM as a selection step which guarantees a strategy matrix with all column norm 1. Practically any matrix can be made to satisfy this condition by scaling the columns.\par  

Likewise in practice we consider an approximate HDMM Waterfilling Mechanism. In this approximate version we do not use strict angular equality to test for membership in a bucket but instead use an approximate version where queries that vary slightly may be put in the same bucket. This is done primarily to account for numerical errors that may arise during the optimization step in HDMM. When using this approximate version of angular equality for queries we lose the provable guarantee of the Sharing Incentive and Non-Interference. However we show that in practice the Waterfilling Mechanism still satisfies all the desiderata so long as the allowed deviation for queries is not too large.  \par 

Mechanisms of this class have two main benefits. First the selection step can be done by any pre-existing algorithm to select representative workloads such as the HDMM selection step or the Matrix Mechanism selection step. This does not hold for Collect First mechanisms as the selection mechanism must be altered to support multiple analysts and workloads. The second benefit is that the Waterfilling Mechanisms allow for budget to be allocated directly to representative queries to satisfy desiderata such as the Sharing Incentive and Non-Interference as opposed to relying on an optimization task to allocate budget appropriately. Like Independent and Workload Agnostic Mechanisms, Waterfilling Mechanisms can provably satisfy both the Sharing Incentive and Non-Interference. \par 



% old proofs

Let $\bm{A}$ be the strategy queries produced by a Waterfilling Mechanism for $k-1$ analysts and $\bm{A'}$ be the strategy queries for $k$ analysts (adding one from previous case). The $i$th analyst is entitled to $s_i\epsilon$ of the budget.
 
 \begin{lemma}
\label{Lemma:sensitivity}
Given the L1 norm of every column of $\mA_i \in \gA$ is 1, the introduction of an additional analyst with weight $s_i$ to the collective of a waterfilling mechanism can only increase the sensitivity of the query set by $s_i$, written formally in Equation~\ref{eq:wf_sensitivity}.
\begin{equation}
    \norm{\bm{A'}}_1 =  \norm{\bm{A}}_1 +s_i
\label{eq:wf_sensitivity}
\end{equation} 
\end{lemma}
\begin{proof}
When a new analyst is added to the collective, for each of their queries, either the mechanism creates a new bucket or the query is added to an existing bucket. If the former, that query becomes a representative and thus is an explicit part of the final strategy query set, adding exactly its sensitivity to the overall sensitivity. If the latter, then the weight of the corresponding bucket increases by the weight of the query, therefore increasing the overall sensitivity by the weight of that query. Since the weight of all of an analysts' queries must equal their overall weight the increase in sensitivity is equal to the overall weight of the analyst.
\end{proof}

\begin{lemma}
 Let $\mA(j)$ be the strategy matrix produced by a Water-filling Mechanism for all analysts up to $j$. Let $\mA(0)$ be the zero matrix. We then have for any $j$, L1 norm of every column of $\mA(j)$ equals to $\sum_{i=1}^j s_i$.
Thus, for every $j$,
\begin{equation}
    \|\mA(j)\|_1 = \sum_{i=1}^j s_i
\end{equation}
\end{lemma}
\begin{proof}
Assume the L1 norm of every column of $\mA(j-1)$ equals to $\sum_{i=1}^{j-1} s_i$.
To get $\mA(j)$, we need to add the queries in $\mA_j$. which increases the sensitivity by $s_j$. Therefore by induction since $A(0)$ has a sensitivity of $0$, $A(j)$ has a sensitivity $\sum_{i=1}^j s_i$ for any $j$.
\end{proof}



% old proof section

\begin{proof}


\begin{definition}
 For any matrix $\mM$, We define $\cnorm(\mM)$ as a vector where the $i$th entry is the L1 norm of the $i$th column of $\mM$, formally
 \begin{equation}
     \cnorm(\mM) = \sum_{\vv\in\mM} |\vv|,
 \end{equation}
 where $\vv$'s are the row vectors of $\mM$ and $|\vv|$ is the vector which takes entry-wise absolute value of $\vv$.
\end{definition}

In Alg.~\ref{alg:waterfilling}, since all weights are positive, $f_B(\ve)$ is positive for all $\ve$. Thus, particularly for $\mA$,
\begin{equation}
    \cnorm(\mA) = \sum_{\vv\in\mA} |\vv| = \sum_{\ve\in B}|f_B(\ve)\ve| =\sum_{\ve\in B}f_B(\ve)|\ve| .
    \label{eqn:water_strategy_bucket}
\end{equation}
Consider adding a query $\vv'$ to $B$ and let the resulting set of buckets $B'$. Let $\ve' = \vv'/\|\vv'\|$ according to Alg.~\ref{alg:waterfilling}. If $\ve'\in B$, $f_{B'}(\ve') = f_B(\ve')+\|\vv'\|$. Otherwise, we add $\ve'$ to $B'$ with $f_{B'}(\ve') = \|\vv'\|$. In both case,
\begin{equation}
    \sum_{\ve\in B'}f_{B'}(\ve)|\ve| = \sum_{\ve\in B}f_{B}(\ve)|\ve| + \|\vv'\||\ve'| = \sum_{\ve\in B}f_{B}(\ve)|\ve| + |\vv'|.
    \label{eqn:water_add_query}
\end{equation}
\begin{lemma}
Consider adding an analyst with strategy matrix $\mA_i$ and weight $s_i$. If the L1 norm of every column of $\mA_i$ is 1, the sensitivity of the resultant strategy queries will increase by $s_i$, formally
\begin{equation}
     \|\mA'\|_1 =  \|\mA\|_1+s_i,
\end{equation}
where $\mA$ and $\mA'$ are the resultant strategy matrix before and after adding this analyst.
\label{Lemma:water_sensitivity}
\end{lemma}
\begin{proof}
In this process, we add $s_i\mA_i$ to $B$ resulting in $B'$. From \cref{eqn:water_strategy_bucket} and \cref{eqn:water_add_query} we get,
\begin{equation}
\begin{split}
    \cnorm(\mA') &= \sum_{\ve\in B'}f_{B'}(\ve)|\ve| = \sum_{\ve\in B}f_{B}(\ve)|\ve| + \sum_{\vv\in s_i\mA_i}|\vv|\\ &= \cnorm(\mA)+\cnorm(s_i\mA_i).
\end{split}
\end{equation}

Given the L1 norm of every column of $\mA_i \in \gA$ is 1, we have $\cnorm(s_i\mA_i) = s_i\vone$, where $\vone$ is a all-one vector. Since the L1 norm of a matrix is the maximum of all L1 column norms, we have
\begin{equation}
\begin{split}
    \|\mA'\|_1 &= \max(\cnorm(\mA')) = \max(\cnorm(\mA)+s_i\vone)\\ &= \max(\cnorm(\mA))+s_i = \|\mA\|_1+s_i
\end{split}
\end{equation}
\end{proof}
Since we can consider the strategy matrix with no analysts as the zero matrix, 
and adding an additional analyst adds their weight to the sensitivity, the L1 norm for the strategy matrix for $k$ analysts is 
\begin{equation}
    \|\mA\|_1 = \sum_{i=1}^k s_i
\end{equation}

Since the ith analyst is entitled to $s_i\epsilon$ of the budget and the sensitivity of the strategy query set is equal to the sum of each analysts' weights then the scale of the noise used to answer the query set is the same regardless of the number of analysts in the collective. Let $x$ be any arbitrary number of analysts The scale of the noise added to each query in the set is as follows. 
\begin{equation}
    \frac{\norm{\bm{A}}_1}{\epsilon} = \frac{\sum_{i=1}^x s_i}{\sum_{i=1}^x s_i \epsilon} = \frac{1}{\epsilon}
\end{equation}
Since the amount of noise being added to each query in the final strategy is the same the amount of error experienced by each analyst is only dependent on the frobenius norm term of the error formula.
For this section of the proof we rely heavily on the following property of the pseudo inverse. 
\begin{theorem}[\cite{pseudo-inverse}] \label{Thrm:Pseudo-inverse}
for any satisfiable linear system $\mathbf{BA} =\mathbf{W}$, $\mathbf{WA^+}$ is a solution to the linear system and $\left\|\mathbf{WA^+}\right\|_F \leq \left\|\mathbf{B}\right\|_F$ for any solution $\mathbf{B}$ to the linear system.
\end{theorem}

We first note that adding a new analyst to the collective results in a change to the overall strategy matrix that can either be expressed by multiplying it by some diagonal matrix with all entries greater than 1 (adding weight to a bucket) or by adding additional rows (creating new buckets). We show below that either of these operations results in a frobenius norm term that is no greater than the term with the original strategy matrix.
\begin{lemma}
For any workload $\mathbf{W}$ and any strategy $\mathbf{A}$ $$\left\| \mathbf{W(DA)^+}\right\|_F \leq \left\| \mathbf{WA^+}\right\|_F   $$ where $\mathbf{D}$ is a diagonal matrix with all diagonal entries greater than or equal to 1 and $\mathbf{A}$ is a full rank matrix.
\end{lemma}
\begin{proof}
We first note that since $\mathbf{D}$ is a diagonal matrix with all entries greater than or equal to 1 then $\mathbf{D^{-1}}$ is a diagonal matrix with all values less than or equal to 1. Since this matrix cannot increase the value of any entry of any matrix multiplied by it the following holds. $$ \left\|\mathbf{WA^+D^{-1}} \right\|_F \leq \left\|\mathbf{WA^+} \right\|_F $$
We then note that $\mathbf{WA^+D^{-1}}$ is a solution to the linear system of equations $\mathbf{B(DA) = W}$.
However since $\mathbf{WA^+D^+}$ is a solution to the linear system of equations then by \cref{Thrm:Pseudo-inverse} the following holds. $$\left\|\mathbf{W(DA)^+} \right\|_F \leq \left\|\mathbf{WA^+D^{-1} }\right\|_F \leq \left\| \mathbf{WA^+}\right\|_F $$
\end{proof}

\begin{lemma}
Let $\mathbf{\tilde{A}}$ be the original strategy matrix $\mathbf{A}$ with additional queries (rows) added to it. We can write this as a block matrix as  $ \mathbf{\tilde{A}}  = \begin{bmatrix}
\mathbf{A} \\
\mathbf{C}
\end{bmatrix} $ 
Where $\mathbf{C}$ are the additional queries.
For any workload $\mathbf{W}$ and any strategy $\mathbf{A}$
$$ \left\| \mathbf{W\tilde{A}^+} \right\|_F \leq \left\| \mathbf{WA^+} \right\|_F $$
\end{lemma}
\begin{proof}


Let $\mathbf{\hat{A}}$ be the original matrix $\mathbf{A}$ padded with additional rows of zeros in order to be the same size as $\mathbf{\tilde{A}}$ written in block matrix form as $ \mathbf{\hat{A}}  = \begin{bmatrix}
\mathbf{A} \\
\mathbf{0}
\end{bmatrix}$.
We note that by the formula for block matrix pseudo-inverse the pseudo-inverse of $\mathbf{\hat{A}}$ is as follows. $\mathbf{\hat{A}}^+  = \begin{bmatrix}
\mathbf{A^+} & \mathbf{0}
\end{bmatrix}$
We then note that $\mathbf{W\hat{A}^+}$ is a solution to the linear system of equations as follows.

\begin{equation} \label{eq1}
\begin{split}
\bf{W\Hat{A}^+\tilde{A}} & = \bf{W \begin{bmatrix}
\bf{A}^+ &
\bf{0}
\end{bmatrix}\begin{bmatrix}
\bf{A} \\
\bf{C}
\end{bmatrix}} \\
 & =\bf{WA^+A} \\
& = \bf{W}
\end{split}
\end{equation}

Therefore since $\mathbf{W\hat{A}^+}$ is a solution to the linear system of equations by \cref{Thrm:Pseudo-inverse} we get the following. $$\left\| \mathbf{W\tilde{A}^+} \right\| \leq \left\| \mathbf{W\hat{A}^+} \right\|_F = \left\| \mathbf{WA^+} \right\|_F $$
\end{proof}
Therefore since both multiplying by a diagonal matrix with all entries greater than 1 and adding additional rows cannot increase the Frobenius norm any combination of the two cannot increase the Frobenius norm. As such any changes to the strategy introduced by adding a new analyst to the collective cannot increase the frobenius norm term of the expected error formula. Likewise since the frobenius norm term of the expected error formula can only decrease and the other terms remain constant when adding a new analyst, adding a new analyst to the collective can only decrease the expected error of each analyst.
\end{proof}


%old lin alg theorem
For this section of the proof we rely heavily on the following property of the pseudo inverse. 
\begin{theorem}\label{Thrm:Pseudo-inverse}
for any satisfiable linear system $\mathbf{BA} =\mathbf{W}$, $\mathbf{WA^+}$ is a solution to the linear system and $\left\|\mathbf{WA^+}\right\|_F \leq \left\|\mathbf{B}\right\|_F$ for any solution $\mathbf{B}$ to the linear system. \cite{pseudo-inverse}
\end{theorem}

%old proof of waterfilling 
In a Waterfilling mechanism we can represent the addition of any  number of new analysts to an existing collective as a modification to the strategy matrix outputted for the existing collective. This modification can be done by first scaling up the existing queries in the strategy matrix and then adding new queries to the strategy matrix. By \cref{lemma:diagonal} and \cref{lemma:rows} these two transformations result in a frobenius norm term that is ether the same or less. By \cref{Lemma:water_sensitivity} the addition of a new analyst results in the other two terms in \cref{eqn:error} remaining constant. Therefore adding any number of new analyst to the collective results in equal or less error therefore satisfying both \cref{eqn:prf1} and \cref{eqn:prf2}.

\begin{equation}
\begin{split}
\Err_i\left(\gM, \gW \cup W_j, \left[\sum_{l: W_l in \gW}s_l + s_j\right] \epsilon\right) & = \frac{2}{\left(\left[\sum_{l: W_l in \gW}s_l + s_j\right]\epsilon\right)^2}\left(\sum_{l: W_l in \gW}s_l + s_j\right) \norm{\bf{W_i(D\tilde{A})^+}} \\
 & =\norm{\bf{W_i(D\tilde{A})^+}} 

\end{split}
\end{equation}


% attempt one at the thing


\begin{equation}
\begin{split}
\Err_i\left(\gM, \gW \cup W_j, \left[\sum_{l: W_l \in \gW}s_l + s_j\right] \epsilon\right) &  \\
= \frac{2}{\epsilon^2}\norm{\bf{W_i(D\tilde{A})^+}}_F^2 & \text{by \cref{eqn:noise}} \\
\leq \frac{2}{\epsilon^2}\norm{\bf{W_i\tilde{A}^+}}_F^2& \text{by \cref{lemma:diagonal}} \\ 
\leq \frac{2}{\epsilon^2}\norm{\bf{W_iA^+}}_F^2& \text{by \cref{lemma:rows}} \\
= \Err_i\left(\gM, \gW, \left[\sum_{l: W_l \in \gW}s_l \right] \epsilon\right) &
\end{split}
\end{equation}

%attempt two at the thing

%old authors line
\author{David Pujol}
\affiliation{%
  \institution{Duke University}
  \city{Durham}
  \state{NC}
  \country{United States}
  \postcode{27708}
}
\email{dpujol@cs.duke.edu}

\author{Yikai Wu}
\affiliation{%
  \institution{Duke University}
  \city{Durham}
  \state{NC}
  \country{United States}
  \postcode{27708}
}
\email{yikai.wu@duke.edu}

\author{Brandon Fain}
\affiliation{%
  \institution{Duke University}
  \city{Durham}
  \state{NC}
  \country{United States}
  \postcode{27708}
}
\email{btfain@cs.duke.edu}

\author{Ashwin Machanavajjhala}
\affiliation{%
  \institution{Duke University}
  \city{Durham}
  \state{NC}
  \country{United States}
  \postcode{27708}
}
\email{ashwin@cs.duke.edu}

%old pathological experiments, removed for space 

\subsection{Pathological Settings}
The next set of experiments uses pathological settings, where we purposely constructed sets of workloads to detect whether our mechanisms violates the Sharing Incentive and Non-Interference. We design this experiment with the intuition that if the the uncommon workload only provides a small proportion of privacy budget but requires a large change in the strategy, the analysts with the common workload will suffer. For example strategies that work well for the total workload perform badly when used to answer the identity workload. Therefore when $k-1$ analysts ask the total workload and the $k$th analyst asks the the identity workload the strategy chosen by the mechanism must change drastically to adjust for the $k$th analyst and therefore reduce the overall utility of the $k-1$ analysts. %This is verified as both Utilitarian and Weighted Utilitarian violate Non-Interference for all $k \geq 3$ in identity-total setting.

In the experiment, every set of workloads consists of 1 uncommon workload and $k-1$ common workloads. We experimented on 3 types of workloads: Singleton, Identity, and Total. We fixed the size of data $n=16$ and tried different values of $k \in [2,10]$.

We present the results for 1 identity workload with $k-1$ total workload (identity-total) in \cref{fig:adv}, since it can best show the violation of the Sharing Incentive and Non-Interference. Since Independent and Identity mechanism both trivially satisfy these 2 properties, we only present results for Utilitarian HDMM, Weighted Utilitarian HDMM and HDMM Waterfilling mechanism.
%Unfortunately, all mechanisms except Independent HDMM violate Non-Interference in some cases. AEgal, MEgal and WUtil  violate Non-Interference when 1 analyst asks the Total workload and $k-1$ ask the  Identity  workload with $k \geq 3$. Utilitarian violates Non-Interference for 1 Identity and $k-1$ Total with $k \geq 2$. Violations are also observed for combinations of All Range and Total.
\begin{figure}[th]
  \begin{subfigure}[b]{0.495\linewidth}
    \centering
    \includegraphics[width=1\linewidth]{fig/adv_max_ratio_errors_k2.pdf}
    \caption{Max Ratio Errors ($k=2$)}
    \label{fig:adv_ratio}
  \end{subfigure}%%
  \begin{subfigure}[b]{0.5\linewidth}
    \centering
    \includegraphics[width=1\linewidth]{fig/adv_inters_k10.pdf}
    \caption{Empirical Interference ($k=10$)}
    \label{fig:adv_inter}
  \end{subfigure}
  \caption{Maximum Ratio Errors and Empirical Interference incurred by mechanisms in pathological settings. Values greater above 1 signify a violation of the Sharing Incentive and Non-Interference respectively. $k$ is the number of analysts.}
  \label{fig:adv}
\end{figure}

\cref{fig:adv_ratio} shows that only Utilitarian violates the Sharing Incentive and the violation is significant. \cref{fig:adv_inter} shows both Utilitarian and Weighted Utilitarian violates Non-Interference and the violation of Utilitarian is much more significant. Waterfilling mechanism satisfies both of them as expected.


% STARTING REVISIONS HERE 

% OLD PRACTICAL SETTINGS
\subsection{Practical Settings}
\label{sec:prac}
\input{experiment_figure}
We generate practical settings using a series of random steps using the census example workloads provided in \cite{HDMM}. We tested on the race workloads with \new{domain} size $n=64$.
\begin{enumerate}
    \item We first fix the dataset size $n$. We then generate the number of analysts by picking an integer $k$ uniformly random from $[2, k_{\max}]$. We let the number of analysts be $k$. \new{Each analyst is given equal weight}.
    \item Each analyst then pick a workload uniformly random from the set of 8 workloads, including 3 race workloads, Identity, Total, Prefix Sum, H2 workload, and custom workload.
    \item If they get custom workload, we chose their matrix size by picking an integer uniformly random from $[1, 2n]$.
    \item For each query in matrix we chose a class of query uniformly sampled from the set including range queries (0-1 vector with contiguous entries), singleton queries, sum queries (random 0-1 vector) and random queries (random vector). The query is thus a random query within its class.
    \item The custom workload is thus a vertical stack of the queries.
    \item We repeat this procedure $t$ times to get $t$ randomly chosen sets of workloads. We call them $t$ instances.
\end{enumerate}

 We present the results for $k_{\max}=20$ as a representative in \cref{fig:prac}. The figure is a box plot of $t=100$ instances is generated randomly using the above procedure. The green line represents the median and the green triangle represents the mean. The box represents  the 25th percentile to the 75th percentile.
%We experimented on other $k_{\max}$ from 5 to 30 and the results are qualitatively similar. We also experimented on a workload set without census workloads and they give qualitatively similar results.
\cref{fig:prac_total} gives an overall view of the efficiency of different mechanisms. As expected, Utilitarian HDMM, a mechanism optimized for overall error, performs the best. Meanwhile Independent HDMM, a mechanism which does not utilize the group structure of the problem at all performs the worst. The other three mechanisms have similar errors and are not much worse than Utilitarian HDMM. 

%It is important to note that the identity strategy only performs well since the practical workloads which we sample from are mostly sparse and easy to answer using the Identity strategy. This will not always be the case.
%Weighted Utilitarian HDMM is the best among the other three, followed by Identity mechanism and then Waterfilling mechanism. All of them are not much worse than Utilitarian HDMM.

\cref{fig:prac_ratio} shows how other mechanisms compared with Independent HDMM in terms of maximum ratio error among all analysts. Utilitarian HDMM violates the Sharing Incentive in a small number of instances as there are some outliers with maximum ratio error larger than 1. Weighted Utilitarian and The Waterfilling mechanism satisfied the Sharing Incentive. Although Identity also has some outliers larger than 1, since independent HDMM is not the independent form of this mechanism it does not violate the Sharing Incentive.

%However, since the error from identity is independent of the other analysts choices any analyst who receives poor error under Identity will receive that same poor error regardless of the number of analysts or their workloads. These analysts are arbitrarily punished by the mechanism since it cannot adapt to any analysts' needs. This demonstrates how violating Adaptivity makes Identity undesirable.

\cref{fig:prac_inter} gives an empirical indication on whether a mechanism satisfies Non-Interference in practical settings. It can be seen that both Utilitarian and Weighted Utilitarian HDMM violate Non-Interference in some cases. Weighted Utilitarian has fewer instances which violate Non-Interference than Utilitarian. The Weighted Utilitarian mechanism also violates Non-Interference to a smaller extent than the Utilitarian Mechanism. The other three mechanisms do not violate Non-Interference as we expect.

From our experiment results, we can see that our HDMM Waterfilling mechanism have achieved our main goal of providing a mechanism which satisfies all three desiderata while maintaining high utility. It is also worth noting that Weighted Utilitarian HDMM also satisfies the Sharing Incentive empirically and can provide a higher utility with only small violations of Non-Interference.

% OLD EXPERIMENTAL SETUP
\subsection{Experimental Setup}
We designed experiments to both test if the mechanisms proposed satisfy the desiderata as well as how they perform in practice.
 For the following experiments we use HDMM \cite{HDMM} as the selection step, but any selection step can be used in practice. As HDMM is a variant of the matrix mechanism (MM) \cite{Matrix10}, the mechanism is data independent for linear queries and the expected error of the matrix mechanism can be analytically calculated for any given strategy matrix. In addition, we can consider the Identity Mechanism a variant of matrix mechanism with a fixed identity strategy matrix $\mI$, $\MM(\mI)$.
We note some commonly used workloads and their corresponding workload matrices $\mW$ in \cref{tab:common_workloads}.
\begin{table*}[ht]
\caption{Common workloads used for \new{domain} size $n$}
\begin{tabularx}{\textwidth}{|l|l|X|}
\hline
\textbf{Workload} & \textbf{Description} & \textbf{Matrix} \\ \hline
Identity & Histogram on all $n$ categories & $n\times n$ identity matrix $\mI_n$ \\ \hline
Total & The sum of all $n$ categories & $1\times n$ all-ones row matrix $\mT_n$ \\ \hline
Singleton & One single category & $1\times n$ row matrix $\mS_{n,i}$ with 1 in the $i$th entry and 0 in other entries \\ \hline
Prefix Sum & The prefix sum of all $n$ categories & $n\times n$ lower triangular matrix of ones $\mP_n$ \\ \hline
H2 workload  & Hierarchical matrix $\gH^2$ & $(2n-1)\times n$ matrix: vertical stack of $\mI_{n/t}\otimes \mT_{t}$ for $t = 1,2,4, \ldots, n$ \\ \hline
\end{tabularx}%
\label{tab:common_workloads}
\end{table*}

In addition, The Waterfilling mechanism has a tolerance parameter $\tau$. We experimented with several values of $\tau$. Results shown in \cref{sec:Experiments_Tolerance} and found $\tau = 0.001$ is a value that achieves good overall accuracy. As such we set it to be $0.001$ in all our experiments.

For the figures, each workload is given an abbreviations as follows: Ind (Independent HDMM), Iden (Identity mechanism), Util (Utilitarian HDMM), WUtil (Weighted Utilitarian HDMM), and Water (HDMM Waterfilling mechanism). For each experiment we run the optimization 10 times and pick the strategy with the minimum loss. Since HDMM is data independent the experiments do not require a particular dataset.

% OLD Marginal workloads

\subsection{Marginal Workloads}
\label{sec:Experiments_Marginal}
We also experiment on another common type of workloads, marginals. For a dataset with $d$ attributes with domain size $n_i$ for the $i$th attribute, we can define a $m$-way marginal as the follows. Let $S$ be a size $m$ subset of $\{1,2,\ldots,d\}$, we can express the workload as the Kronecker product $\mA_1 \otimes \mA_2 \otimes \ldots \otimes \mA_d$, where $\mA_i = \mI_{n_i}$ if $i \in S$ and $\mA_i = \mT_{n_i}$ otherwise. Here $\mI_{n_i}$ is the identity workload matrix and $\mT_{n_i}$ is the total workload matrix. Specifically, a 0-way marginal is the Total workload and a $d$-way marginal is the Identity workload. Also, since there are $\binom{d}{m}$ size-$m$ subset of $\{1,2,\ldots,d\}$, there are $\binom{d}{m}$ different $m$-way marginals. In our experiments for simplicity, we use $d$ attributes all with domain size 2. We repeat the process for generating analyst workloads from \cref{sec:prac} however in this case each individual analyst chooses a workload uniformly at random from the set of set of $\binom{d}{m}$ $m$-way marginals.

%Similar to Step 1 and 2 in the practical setting in \cref{sec:prac}, the detailed experiment procedure is as follows. We first fix $d$, $m$, and the maximum number of analysts $k_{\max}$. We then generate the number of analysts by picking an integer $k$ uniformly random from $[2,k_{\max}]$. We let the number of analysts be $k$. Each analyst then pick a workload uniformly random from the set of $\binom{d}{m}$ $m$-way marginals.

in \cref{fig:prac} we show the results for $1$-way marginal with $d=8$, $k_{\max}=20$, and $n =256$. This figure also contains 100 instances. In particular, there are $d$ 1-way marginals each corresponds to an attribute. For the 1-way marginal with attribute $i$, it consists of 2 queries, where one is the total query with predicate attribute $i$ equals to 0, and the other is with predicate attribute $i$ equals to 1.

\cref{fig:marginal_total} shows Identity mechanism performs worse than the Waterfilling mechanism and both Utilitarian mechanisms. The addition of the 1-way marginals drastically increases the error of identity compared to that of the other mechanisms. This is an example where the Identity perform poorly with regard to total error for a common type of workloads. This is also observed for 1-way marginals with $d=6,7,9,10$. 

%Although there are  workloads where Identity mechanism performs well, the Adaptivity of other mechanisms allow them to be suitable for most cases. Identity mechanism thus should be only used when the data curator has the prior knowledge that workloads analysts tend to ask are all good with Identity mechanism.

\cref{fig:marginal_ratio} and \cref{fig:marginal_inter} are qualitatively similar to those in the practical settings. The Waterfilling Mechanism continues to satisfy all the desiderata while maintaining lower error than the Independent and Identity Mechanisms. Both Utilitarian mechanisms achieve lower overall error but at the cost of violating non interference.

% OLD TOLERANCE FOR WATERFILLING
\subsection{Tolerance for Water-filling Mechanism}
\label{sec:Experiments_Tolerance}
The Water-filling mechanism provably satisfies Sharing Incentive and Non-interference when the tolerance parameter $\tau=0$. However, if we set $\tau =0$ exactly or very small, very similar queries (which may be the same query ideally but are different due to numerical errors in optimizations) will not be combined. This can lead to a large expected error.
On the other hand, a too large $\tau$ may make Water-filling mechanism violate the Sharing Incentive or Non-Interference because queries which are significantly different may be put into the same bucket.

To examine the effect of tolerance in practice, we experimented on different values of tolerance $\tau$ for the HDMM Water-Filling mechanism. \cref{fig:tol} shows the case when $\tau \in [0.1, 0]$, which we consider a reasonable range of the tolerance. The workloads used are 1-way marginals as defined in \cref{sec:Experiments_Marginal}.

\cref{fig:tol_total} shows that the total error is large at both ends, $\tau =0.1$ and $\tau =0$. The total error is the smallest for $\tau=0.01$ and is also small for $\tau = 10^{-3}$ and $\tau=10^{-4}$. This shows that there is no simple relation between the value of tolerance and total errors and we should not set $\tau=0$ exactly in practice. \cref{fig:tol_ratio} shows the violation of Sharing Incentive when $\tau =0.1$ and $\tau=0.01$. From this result, we see that $\tau=0.01$ is too large and $\tau=10^{-3}$ (our default setting) is reasonable. We do not observe violation of Non-interference for all these values of tolerance.
\begin{figure}[ht]
  \begin{subfigure}[b]{0.51\linewidth}
    \centering
    \includegraphics[width=1\linewidth]{fig/tol_marginal_total_errors.pdf}
    \caption{Total Errors}
    \label{fig:tol_total}
  \end{subfigure}%%
  \begin{subfigure}[b]{0.49\linewidth}
    \centering
    \includegraphics[width=1\linewidth]{fig/tol_marginal_max_ratio_errors.pdf}
    \caption{Max Ratio Errors}
    \label{fig:tol_ratio}
  \end{subfigure}
  \caption{Total Errors and Maximum Ratio Errors for 1-way marginals using our HDMM Water-filling mechanism with different values of tolerance $\tau$ (x-axis). Values of maximum ratio error above 1 signify a violation of Sharing Incentive.}
  \label{fig:tol}
\end{figure}
%We also experimented on randomly generated practical queries as defined in \cref{sec:prac}. In that case, we did not observe violation of Sharing incentive but there is violation of non-interference when $\tau\geq 0.01$. There is still no simple relation between $\tau$ and total errors. This also suggests that we should use $\tau\leq 10^{-3}$.

%This experiment shows that $\tau=10^{-3}$ achieves good overall accuracy without violations of Sharing Incentive and Non-interference. We thus use it in our experiments. In practice, we suggest a $\tau = 10^{-3}$ or slightly smaller, but not exactly equals to 0. 


% OLD data-dependent 
\subsection{Data-dependent Non-linear Queries} \label{sec:experiments_nonlinear}
\begin{figure*}[ht]
\resizebox{1\textwidth}{!}{%
	\centering
	\begin{subfigure}[b]{0.308\linewidth}
		\includegraphics[width=1\textwidth]{fig/data_total_errors.pdf}
		\caption{Total Errors (log scale)}
		\label{fig:data_total}
	\end{subfigure}
	\begin{subfigure}[b]{0.254\linewidth}
		\includegraphics[width=1\textwidth]{fig/data_total_errors_2.pdf}
		\caption{Total Errors (zoomed in)}
		\label{fig:data_total_zoom}
	\end{subfigure}
	\begin{subfigure}[b]{0.217\linewidth}
		\includegraphics[width=1\textwidth]{fig/data_max_ratio_errors.pdf}
		\caption{Max Ratio Errors}
		\label{fig:data_ratio}
	\end{subfigure}
	\begin{subfigure}[b]{0.223\linewidth}
		\includegraphics[width=1\textwidth]{fig/data_inters.pdf}
		\caption{Empirical Interference}
        \label{fig:data_inter}
    \end{subfigure}%
}
\caption{Total Errors, Maximum Ratio Errors and Empirical Interference for non-linear queries. Errors shown are empirical expected errors calculated using real data. Values of maximum ratio error and empirical interference above 1 signify a violation of the Sharing Incentive and Non-Interference respectively.}
\label{fig:data}
\end{figure*}
In previous experiments, all workloads are linear and the expected error can thus be calculated without data. Our mechanisms can also be used for non-linear queries. We now experiment on some non-linear queries including \emph{mean}, \emph{medium}, and \emph{percentiles} based on a histogram.

Error in this case is data-dependent and needs to be empirically calculated using real datasets. We use the Census Population Projections \cite{census_population}. The dataset is Population Changes by Race. We choose year 2020 and Projected Migration for Two or more races. This dataset can show the difference between mechanisms clearly. The size of data is $n=86$, representing ages from 0 to 85.

As in the previous 2 experiments, the experiment procedure is as follows. We fix the maximum number of analysts $k_{\max}$. We then generate the number of analysts by picking an integer $k$ uniformly random from $[2,k_{\max}]$. We let the number of analysts be $k$. Each analyst then picks a query uniformly random from the set of 4 queries, including \emph{mean}, \emph{medium}, \emph{25-percentile}, and \emph{75-percentile}. \emph{Mean} is reconstructed from the workload containing the Total query $\mT_n$ and the weighted sum query, a vector representing the attribute values (0 to 85 in our case). \emph{Medium} and \emph{percentiles} are reconstructed from the Prefix Sum workload $\mP_n$. The expected error here is the mean squared error of 10000 samples calculated using the Laplace mechanism.

In \cref{fig:data} we show the results of 100 instances (sets of queries) with $k_{\max}=20$. \cref{fig:data_total} shows that the Independent mechanism performs much worse than all other mechanisms in terms of total error. \cref{fig:data_total_zoom} is the zoomed in version of \cref{fig:data_total}, removing Independent. Since the answer of a non-linear query is reconstructed using the result of a different linear workload, Utilitarian is not guaranteed to have the lowest total errors. We can see that Weighted Utilitarian outperforms Utilitarian here. The other two mechanism have higher total errors, and the Waterfilling mechanism has a better median total errors than Identity.

\cref{fig:data_ratio} and \cref{fig:data_inter} shows the max ratio errors and empirical interference. Since Independent and Identity mechanism satisfy the Sharing Incentive and Non-Interference by definition, we omit them here. We can see that all 3 other mechanisms satisfy the Sharing Incentive as they all have max ratio errors smaller than 1. Both Utilitarian mechanisms violate Non-Interference as shown in \cref{fig:data_inter}. Waterfilling mechanisms satisfies Non-Interference. The outliers are due to numerical errors since we are using empirical expected errors instead of analytical ones.

These results show that our mechanisms are also good for non-linear queries and have similar properties as the instances with linear queries. The results are qualitatively similar for $k_{\max}=10$.

%part of response letter draft one 


\item \textbf{D1:}  We are not aware of any variant of the matrix mechanism which can take into account prior knowledge into the optimization. As far as we are aware this remains a challenging open problem which is outside the scope of this paper. This is an interesting approach however the simple algorithm provided as stated is under-defined. Using the reviewers rubric we were able to construct two mechanisms, one which did not outperform the baseline and another which failed to satisfy the desiderata. The algorithms are as follows.
    
\begin{algorithm}[h]
\SetAlgoLined
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
Order the agents from greatest to least $\epsilon_i$ \\
\For{each agent $i$}{
    \eIf{$W_i = W_j$ where $j < i$ }{
    Answer $W_i$ using the answers from $W_j$}
{Answer $W_i$ with the matrix mechanism using $\epsilon_i$}
}
 \caption{}
\end{algorithm}

\begin{algorithm}[h]
\SetAlgoLined
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
Order the agents from greatest to least $\epsilon_i$ \\
\For{each agent $i$}{
    \eIf{$W_i$ is inferable from $W_j$ where $j < i$ }{
    Reconstruct the answers to $W_i$ using the answers from $W_j$}
{Answer $W_i$ with the matrix mechanism using $\epsilon_i$}
}
 \caption{}
\end{algorithm}

Consider the scenario where there are two analysts, Alice and Bob. Alice and Bob both ask the exact same workload and each receive the same fraction $\frac{\epsilon}{2}$ of the total privacy budget. In this case Algorithm 1 would publish the answer to the workload using $\frac{\epsilon}{2}$ of the privacy budget. The independent mechanism however would answer both Alice and Bobs workloads separately using $\frac{\epsilon}{2}$ of the privacy budget and publish both, resulting in two samples of the noisy measure from the same distribution which both Alice and Bob can use to infer a more accurate estimate of their workload.

Likewise consider the case where Alice asks the Identity workload and Bob asks the total workload again each analyst receives half of the privacy budget. Algorithm 2 would first answer Alices workload with $\frac{\epsilon}{2}$ of the privacy budget. It would then see that Bobs workload can be reconstructed using the $n$ query answers of Alices workload and instead of answering Bob's workload directly uses those measures instead. In this case Bob recives an answer that contains $n$ samples of noise instead of the one sample of noise he would have recived under the indpendent mechanism therefore violating the sharing incentive. \par 
We have included in \cref{sec:Future_work} a brief discussion on the importance of incorporating prior knowledge for future work.+


% old waterfilling section
\new{One of the main sources of inefficiency in independent mechanisms is that if multiple analysts ask the same query an independent mechanism must answer the query multiple times, using privacy budget each time it does so. The waterfilling mechanism circumvents this by selecting a set of strategy queries for each analyst and then grouping common queries together and pooling privacy budget together to answer said queries.} The mechanism assigns each individual query to a bucket. Buckets represent groups of equivalent queries that can all be answered with a single representative query. In Algorithm~\ref{alg:waterfilling}, Queries are equivalent if they are simple scalar multiples of one another with some deviation bounded by a parameter $\tau$. 


The mechanism generates a  strategy for each analyst using the given selection step. These strategies are then scaled by the weight of each analyst. Those strategies are split into their independent queries. For each of those queries the mechanism assigns a weight (usually each query is given an equal share of the analysts' share of the privacy budget) and finds a bucket with an equivalent representative query to which the query is added. The associated weight of the bucket is also increased by the query's weight. If no bucket with an equivalent representative query exists, then a new bucket is created with the query as the representative and with its associated weight. The mechanism constructs a single joint set of strategy queries by taking the representative query from each bucket and weighting it by the bucket's weight. The joint strategy queries are then measured directly using the Laplace mechanism. \par 
\new{Since the selection step introduces some numerical instability to the algorithm we have added the parameter $\tau$, which determines how much two queries are allowed to deviate and still be assigned to the same bucket. This allows queries which are the same up to some numerical error to be assigned to the same bucket. $\tau$ lies in the range $[0,1]$ where higher values allow for more variability.}
\\If $\tau = 0$ then queries must be scalar multiples of one another to be assigned to the same bucket. 


%old design paradigm figure 




\begin{figure*}[ht]
\resizebox{0.75\textwidth}{!}{%
	\centering
	\begin{subfigure}[b]{0.35\textwidth}
		\includegraphics[width=1\textwidth]{fig/Independentanimation.pdf}
		
		\caption{Independent}\label{fig:independent}
	\end{subfigure}
	\begin{subfigure}[b]{0.35\textwidth}
		\includegraphics[width=1\textwidth]{fig/Workload_agnostic_animation.pdf}
		
		\caption{Workload Agnostic}\label{fig:agnostic}
	\end{subfigure}
}
\resizebox{0.75\textwidth}{!}{%
    \begin{subfigure}[b]{0.35\textwidth}
		\includegraphics[width=1\textwidth]{fig/Collect_first_animation.pdf}
		
		\caption{Collect First}\label{fig:collect}
	\end{subfigure}
	\begin{subfigure}[b]{0.35\textwidth}
		\includegraphics[width=1\textwidth]{fig/Select_first_mechanism.pdf}
		
		\caption{Select First}\label{fig:select}
	\end{subfigure}
}
\caption{\new{Design Paradigms} for Multi-Analyst DP Query Answering}
\label{fig:algos}
\end{figure*}



% single row version

\begin{figure*}[ht]
\resizebox{\textwidth}{!}{%
	\centering
	\begin{subfigure}[b]{0.25\textwidth}
		\includegraphics[width=1\textwidth]{fig/Independentanimation.pdf}
		
		\caption{Independent}\label{fig:independent}
	\end{subfigure}
	\begin{subfigure}[b]{0.25\textwidth}
		\includegraphics[width=1\textwidth]{fig/Workload_agnostic_animation.pdf}
		
		\caption{Workload Agnostic}\label{fig:agnostic}
	\end{subfigure}
	\begin{subfigure}[b]{0.25\textwidth}
		\includegraphics[width=1\textwidth]{fig/Collect_first_animation.pdf}
		
		\caption{Collect First}\label{fig:collect}
	\end{subfigure}
	\begin{subfigure}[b]{0.25\textwidth}
		\includegraphics[width=1\textwidth]{fig/Select_first_mechanism.pdf}
		
		\caption{Select First}\label{fig:select}
	\end{subfigure}

	
}
\caption{\new{Design Paradigms} for Multi-Analyst DP Query Answering}
\label{fig:algos}
\end{figure*}

